The Long Baseline Neutrino Experiment (LBNE) Water Cherenkov Detector (WCD) Conceptual Design Report (CDR)

Conceptual Design Report developed for the Water Cherenkov Detector (WCD) option for the far detector of the Long Baseline Neutrino Experiment.

==> reqtex/req.tex <==
% Requirements definition.  This file is generated, do no edit.

\usepackage{ifthen}
\usepackage{color}

\makeatletter
% \registerRequirement{number}{version}{status}{value}{unit}{text}
\newcommand\registerRequirement[6]{%
  \@namedef{reqVersion-#1}{#2}%
  \@namedef{reqStatus-#1}{#3}%
  \@namedef{reqValue-#1}{#4}%
  \@namedef{reqUnit-#1}{#5}%
  \@namedef{reqText-#1}{#6}%
}
% \requirement[version]{number}{what}
\newcommand\requirement[3][0]{%
  \@ifundefined{req#3-#2}{%
    [whatever else you want to do]
  }{%
    \@nameuse{req#3-#2}%
    \ifthenelse{\equal{#1}{0}}{}{%
      \ifthenelse{\equal{#1}{\@nameuse{reqVersion-#2}}}{}{%
          \textcolor{red}{~(using requirement #2's #3 at version #1, newest is \@nameuse{reqVersion-#2})}%
        }%
      }%
    }%
}
\makeatother

\registerRequirement{1.1}{1}{}{}{}{}
\registerRequirement{1.1.1}{1}{accepted}{}{}{A search for, and precision measurements of, the parameters that govern $\nu_\mu \to \nu_e$ oscillations. This includes measurement of the third mixing angle $\theta_{13}$, for whose value only an upper bound is currently known, and if $\theta_{13}$ is large enough, measurement of the CP violating phase $\delta$ and determining of the mass ordering (sign of $\Delta m^2_{32}$).}
\registerRequirement{1.1.2}{1}{accepted}{}{}{Precision measurements of $\theta_{23}$ and  $\left|\Delta m^2_{32}\right|$ in the $\nu_\mu$ disappearance channel.}
\registerRequirement{1.1.3}{1}{accepted}{}{}{A search for proton decay, yielding a significant improvement in current limits on the partial lifetime of the proton ($\tau$/BR) in one or more important candidate decay modes, e.g. $p \to e^+ \pi^0$ or $p \to K^+ \nu$.}
\registerRequirement{1.1.4}{1}{accepted}{}{}{Detection and measurement of the neutrino flux from a core collapse supernova within our galaxy, should one occur during the lifetime of LBNE.}
\registerRequirement{1.2}{1}{}{}{}{}
\registerRequirement{1.2.1}{1}{accepted}{}{}{Other accelerator-based neutrino oscillation measurements.}
\registerRequirement{1.2.2}{1}{accepted}{}{}{Measurements of neutrino oscillation phenomena using atmospheric neutrinos.}
\registerRequirement{1.2.3}{1}{accepted}{}{}{Measurements of other astrophysical phenomena using medium energy neutrinos.}
\registerRequirement{1.2.4}{1}{accepted}{}{}{Near detector studies of weak interaction}
\registerRequirement{1.2.5}{1}{accepted}{}{}{Near detector studies of nuclear and nucleon structure}
\registerRequirement{1.2.6}{1}{accepted}{}{}{Near detector searches for new physics}
\registerRequirement{1.3}{1}{}{}{}{}
\registerRequirement{1.3.1}{1}{accepted}{}{}{Detection and measurement of the diffuse supernova neutrino flux.}
\registerRequirement{1.3.2}{1}{accepted}{}{}{Measurements of neutrino oscillation phenomena and of solar physics using solar neutrinos.}
\registerRequirement{1.3.3}{1}{accepted}{}{}{Measurements of astrophysical and geophysical neutrinos of low energy}
\registerRequirement{2.0}{1}{}{}{}{}
\registerRequirement{2.10}{1}{}{}{}{The $\nu_e$ content in the beam shall be kept to a minimum.}
\registerRequirement{2.11}{1}{}{}{}{The beam shall be sign-selected to provide separate neutrino and anti-neutrino beams with high purity to enable measurement of CP violation and precision oscillation measurement.}
\registerRequirement{2.12}{1}{}{}{}{The beam shall be aimed at the far detector with an angular accuracy that allows the determination of the far detector spectrum using the near detector measurements.  In this determination the angular accuracy shall not be the dominant factor in the determination of oscillation parameters. }
\registerRequirement{2.13}{1}{}{}{}{Proton beam will be extracted in a single turn from the main injector at the end of an acceleration cycle.}
\registerRequirement{2.14a}{1}{}{}{}{ The far detector shall be located at a depth to reduce the number of in-time (within the beam spill time) cosmic ray background so that it does not contribute more than 1 \% of the final beam neutrino sample. }
\registerRequirement{2.14b}{1}{}{}{}{The far detector shall be located at a depth to reduce the number of in-time (within the beam spill time) cosmic ray background so that it does not contribute more than 1 \% of the final beam neutrino sample. }
\registerRequirement{2.15}{1}{}{}{}{The total number of observed electron-neutrino and electron-antineutrino type events, including background, shall be sufficient to measure the CP phase to better than 3$\sigma$ at maximum CP violation if the value of the third mixing angle is in the accessible range.}
\registerRequirement{2.16}{1}{}{}{}{The near detector shall have sufficient energy, angular and spatial resolution that when combined with the detailed knowledge of the beamline geometry we will obtain a data-driven estimate of the far detector flux and spectrum for muon-neutrinos and muon-antineutrinos separately.}
\registerRequirement{2.17}{1}{}{}{}{The near detector shall measure the electron-neutrino and antineutrino contamination in the beam. The spectrum of this contamination shall be measured with low background.  }
\registerRequirement{2.18}{1}{}{}{}{The near detector shall measure rates of interactions that could mimic signal events in the far-detector nuclear targets.}
\registerRequirement{2.19}{1}{}{}{}{The near detector shall measure spurious asymmetries between neutrino and antineutrino interactions.}
\registerRequirement{2.1a}{1}{proposed}{}{}{Far detector shall be capable of identifying neutrino and anti-neutrino beam events in sufficient numbers within the fiducial volume of the detector and with a single electron particle in the final state with no other visible accompanying particle. The electron energy and direction with respect to the neutrino beam shall be measured.}
\registerRequirement{2.1b}{1}{proposed}{}{}{Far detector shall be capable of identifying electron neutrino and anti-neutrino charged current beam events in sufficient numbers within the fiducial volume of the detector. The neutrino flavor of the event will be identified by clearly identifying the primary final state charged electron. The total energy of the charged current event shall be measured. }
\registerRequirement{2.20}{1}{}{}{}{The near detector shall measure neutrino interactions for each qualified beam pulse per proton on target.}
\registerRequirement{2.21}{1}{}{}{}{The far-detector size multiplied by the duration of operation [expressed in kiloton-years] shall be sufficient to yield a scientifically competitive result on proton decay}
\registerRequirement{2.22}{1}{}{}{}{There shall be good signal to background ratio during a few-tens-of-second burst for a core collapse supernova within 20 kpc (within the Milky Way).}
\registerRequirement{2.23}{1}{}{100.0}{kt}{The far detector shall be of sufficient fiducial volume to allow unambiguous measurement of the diffuse supernova neutrino flux independent of model uncertainties.}
\registerRequirement{2.24}{1}{}{4000.0}{m.w.e.}{The far detector shall be located at sufficient depth to reduce residual muon-induced spallation to below the diffuse supernova neutrino rate over the energy range of interest.}
\registerRequirement{2.25}{1}{}{<1}{event/kt/century}{The far detector shall be capable of reducing atmospheric neutrino-induced physics backgrounds to below the diffuse supernova neutrino rate over the energy range of interest via efficient neutron tagging.}
\registerRequirement{2.26}{1}{}{}{}{The far detector shall be capable of identifying individual diffuse supernova neutrino events as such via efficient neutron tagging.}
\registerRequirement{2.27}{1}{}{}{}{The data acquisition and online system shall be configurable to allow prompt processing of event information on a few-minute timescale to enable a supernova alert in the case of a burst, for a supernova as close as 0.1 kpc.}
\registerRequirement{2.28}{1}{}{}{}{Individual event times shall be measured with at least microsecond accuracy.}
\registerRequirement{2.29}{1}{}{}{}{The detector and data acquisition shall be configured to allow, to the extent possible, continuous running for long periods in order to maintain high (above 90\%) livetime for a supernova.  For a separate/modular detector configuration, provision shall be made to ensure that at least one module can be running at all times.}
\registerRequirement{2.2a}{1}{proposed}{}{}{Far detector shall be capable of identifying neutrino and anti-neutrino beam events in sufficient numbers within the fiducial volume of the detector and with a single muon particle in the final state with no other visible accompanying particle. The muon energy and direction with respect to the neutrino beam shall be measured.}
\registerRequirement{2.2b}{1}{proposed}{}{}{Far detector shall be capable of identifying muon neutrino and anti-neutrino charged current beam events in sufficient numbers within the fiducial volume of the detector and identify the primary muon particle emerging from the main event vertex.  The total energy of the charged current event shall be measured. }
\registerRequirement{2.3}{1}{proposed}{}{}{Far detector shall be capable of identifying events with multiple electromagnetic showers and non-showering particles produced within the fiducial volume of the detector.}
\registerRequirement{2.4a}{1}{proposed}{}{}{Far detector shall be capable of collecting inverse beta decay (IBD) interactions that arrive in a short period of time. In IBD an anti-electron neutrino interacts with a free proton in the detector to produce a positron and a neutron in the final state. IBD events due to supernova are expected to be distributed around 10MeV.}
\registerRequirement{2.4b}{1}{proposed}{}{}{Far detector shall be capable of collecting low energy charged current neutrino interactions on Ar40 nucleus that arrive in a short period of time.The electron shall be detected and its energy measured. Events due to supernova are expected to be distributed around 10MeV. }
\registerRequirement{2.4c}{1}{}{>90\%}{}{Far detector shall have high uptime with little event by event  deadtime to allow the capture of low probability astrophysical events that could occur at any time with no external trigger. }
\registerRequirement{2.5}{1}{proposed}{}{}{Far detector shall be capable of identifying neutrino electron elastic scattering at energies below 20 MeV from a distant neutrino source with good efficiency. The elastic scattering angle is to be measured and it is expected to be less than 25$^\circ$}
\registerRequirement{2.6a}{1}{proposed}{}{}{Far detector shall be capable of efficient tagging of neutrons that are in the final state of IBD interactions.}
\registerRequirement{2.7}{1}{}{}{}{A baseline of sufficient length shall be established between a neutrino beam facility and a far detector facility so that the difference between muon to electron neutrino conversion for the two cases of neutrino mass ordering can be clearly separated from the variation due to the CP phase leading to unique determination of the CP phase. }
\registerRequirement{2.8}{1}{}{}{}{The beam spectrum shall cover the energy region of the first two oscillation maximums affected by muon- to electron-neutrino conversion from the atmospheric parameters. In addition, it should extend beyond to higher energies, to obtain maximum sensitivity to the matter effect, as long as high signal to background is maintained.}
\registerRequirement{2.9}{1}{}{}{}{The neutrino beam spectrum shall be tunable so that beam with both lower average energy (below the first oscillation node) and higher average energy (above 3 GeV) can be achieved without substantial downtime. 
}


==> volume-4-WCD/alt-InWaterElectronics.tex <==
% reviewed by J. Dolph for inclusion in 2011 CDR update


\section{In Water Electronics}
\label{sec:inwater}


An alternative to the reference design electronics
described in Chapter~\ref{ch:elec-readout} is to place the bulk of
the active electronics under the water, very near the PMTs. The major
advantage of such a scheme is that it could significantly reduce the
size of the cable plant traveling up the side of the vessel walls
and, thereby, perhaps, allow a significantly less expensive
installation scheme.
% In this section we will outline a possible
%``In-Water'' architecture, show the availability of commercial
%housings and connectors that could be used in such a scheme, and list
%some of the other possible advantages and disadvantages of the
%``In-Water'' alternative that will be evaluated over the coming
%months. 

The alternate ``In-Water'' solution places the electronics
close to the sensors and connects to the PMTs with short ($<$10 m)
cables. The PMT signals are digitized in the same manner as described
in the reference design, taking advantage of custom integrated
circuits to allow many PMTs (16 to 32) to feed a single high speed
Ethernet data connection. This electronics would be mounted in an
electronics module or capsule. Commercial underwater encapsulation
technology used for deep undersea oil and natural gas exploration and
communication cables could be used to house these electronics and a
number of vendors of such housings, connectors and cables were
identified. A sketch of one such possibility is shown in
Figure~\ref{UWtower}.
\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=3in]{volume-4-WCD/figures/Column.pdf}
  \end{center}
  \caption[In-water electronics layout]{Water Cherenkov detector PMT towers arranged as single
    column (32 PMTs) or dual column (64 PMTs) or quad (128 PMTs) are
    connected via equal length (10 m) cables to readout ASIC and power
    supplies encapsulated in the high density polyethylene (HDPE)
    capsule rated for 500~psi pressure.  }
  \label{UWtower}
\end{figure}
These commercial housings and connectors are typically used in much
more demanding environments than we face, and so little or no R\&D is
required for packaging an underwater solution.

At the schematic level underwater and above water electronics would be
essentially identical with both relying heavily on custom ASICs for
time and charge measurement.  The major advantage of this scheme is
that the multiplexing of data, power and control allows many fewer
cables between the capsule and the surface compared to the reference
design and those connections are all at low voltages and so amenable
to a single multi-conductor cable. For instance, concatenating the
functions of the High Voltage and Readout Boards described in
Chapter~\ref{ch:elec-readout} into a form factor suitable for an
underwater capsule as shown in Figure~\ref{UWblock} could then reduce
the link to the surface to two pairs of Ethernet signals, two pairs of
precision clock and synch signals, one or two pairs of hardware
trigger signals and a pair or two of DC power connections --- one
eight pair low voltage multi-conductor cable in place of sixteen High
Voltage coaxial cables --- a significant reduction in cable volume and
cable plant stiffness. 
\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=6.5in]{volume-4-WCD/figures/InwaterElexBD.pdf}
  \end{center}
  \caption[In-water electronics capsule]{Interior of a high density polyethylene capsule in a block diagram format. Proposed capsule is sized to host underwater connections to serve up to  four PMT columns (128 PMTs).  }
  \label{UWblock}
\end{figure}
Initial investigations into capsules, connectors and cables indicate
that the cost differences between the reference and underwater
schemes are relatively small. 
%Initial estimates of installation costs
%for the PMTs and their cables, on the other hand, are quite
%significant and so it is possible that an alternate configuration of
%the electronics could allow an alternate installation and/or vessel
%liner scheme which could save very significant amounts of money.


A major downside of such a scheme is the loss of access
to the underwater part of the electronics for repair, rework, or
upgrade and, lacking a technical or major cost advantage it is
unlikely that an underwater alternate would be attractive. Another major downside is the heat load from the electronics creating water convection currents that will degrade the water attenuation. 
%However,
%as noted above, the possibility of underwater electronics enabling a
%much simpler alternate PMT mounting and installation scheme,
%thereby, saving very significant sums seems sufficiently plausible at
%the moment that these alternatives are being carried forward into the
%preliminary design phase.

%In addition to the expected reduction in the cable plant, there are a
%number of other possible advantages to the underwater scheme:
%\begin{itemize}
% \item Because the PMT assemblies are connected with short cables to
%   the electronics capsule it is possible to imagine relatively simple
%   modifications or upgrades to the light collection system.

% \item Much less cable above the deck, no significant lengths of
%   stored cable and that small amount of cable could have fire
%   retardant sleeves obviating the need for additional above deck fire
%   protection.
   % Note, not clear you can get away from HDPE jackets and keep the water clean so I don't want to claim non-flammability - at least without a candidate cable.

% \item Significantly fewer huts or racks and less heat load installed
   above the deck. This means that much less HVAC, or water needs to
   be distributed above the deck for cooling. 
%The cooling system for
%   the water plant removes the majority of the heat generated by the
%   experiment.

% \item The material in contact with the water is significantly
   reduced.
%\end{itemize}

%With a vertical installation technique chosen for the reference design, the %following additional
%advantages are possible:
%\begin{itemize}
% \item The wall PMTs and related electronics might be repaired in a
%   short (few day) maintenance period.

% \item A highly parallel installation procedure might be employed to
   minimize the installation time.

% \item In the event that mounts to the wall are not needed a design
   with no vessel and only a liner could be investigated.
%\end{itemize}

%The major disadvantages to in-water electronics are:
%\begin{itemize}
%  \item Even with a vertical installation technique for the walls,
    upgrading or repairing the electronics for the floor and deck PMTs
    would require draining the detector which would represent a
    minimum of a one-year shutdown.
%, unless a different length cabling
%    scheme is adopted. Upgrading is not a very serious concern as the
%    electronics is not the limiting factor in the detector performance
%    --- the detector performance is determined by the light collection
%    system and floor PMTs, for example, constitute only 15\% of the
%    total.

 %\item As the bulk of the underwater electronics is not easily
  accessible, the reliability of the electronics becomes a much more
  serious issue and demonstration and verification of quality control
  will be extremely important.
% The added risk to the project from
%  electronics failures after installation would need to be evaluated
%  in detail.
\end{itemize}

%In summary, the underwater electronics alternative, in conjunction
%with alternative PMT mounting and vessel construction schemes, holds
%out the possibility of significant cost savings in installation labor,
%time and material and so is being actively examined as part of the
%design decision process.


==> volume-4-WCD/calib-gad.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.


%\fixme{AH 7/27 Editedin the context of the Gd chapter). We will keep this information here in the Calib chapter, I think. Here it is. AH needs to reconcile with earlier stuff.

\section{Gadolinium Monitoring (WBS 1.4.5.6)}
\label{sec:v4-gad-mon}

This WBS element will outline the calibration group's responsibilities
and plans for monitoring the gadolinium concentration throughout the
detector volume over the lifetime of the experiment.  Within this
overall task a number of different calibration sources may be used. 
Additionally, it may also be possible to monitor changes with respect
to position and time with naturally occurring neutrons via muon
spallation. 

Eddies and regions of low flow within the detector may generate concentration 
variations in the detector.  We will need to monitor
the gadolinium-capture efficiency at regular intervals in time and
space, using source hatches built into the deck.  A grid of deck
hatches spaced every four meters or so along the $x$ and $y$ axes should be
sufficient to generate a grid of approximately 200 potential locations
within the tank.  From these we can estimate our uncertainty from
neutron-source measurements.  We will require at least one high-intensity, 
physically small and easily deployed source in order to
cover enough grid locations.

\subsection{Neutron Sources}
Three devices are envisioned; a
tagged americium beryllium (Am-Be) source, a californium ($^{252}$Cf) source and a
Deuterium Tritium (DT) source. Each device will be subject to a different set of
systematic uncertainties so that measurements can be cross-checked
against each other.   The concept
is to employ methods that are each affected by an orthogonal set of
systematic effects, advantages and disadvantages, so that results can
be compared and cross checked with simulations to gain as full an
understanding as possible of the one common element in each case (the neutron-capture efficiency). Monte Carlo simulations will be needed to model
each of the sources in order to understand and account for the systematics associated with each source.  

\subsubsection{Americium Beryllium (Am-Be)}
Am-Be sources produce both single neutrons and
neutrons in coincidence with a 4.4~MeV gamma ray.  A small detector,
tuned to detect the gamma ray and deployed with the source, can tag
the presence of the associated neutron.  
Alternatively,
deploying the source together with a scintillating crystal tags the neutron by a different process: 
the detector PMTs detect an extremely bright event when the gamma ray converts to visible light in the scintillator.

Two problems can interfere with this measurement, however. 
First, neutrons emitted by the source may get captured inside the
hardware containing the gamma-ray detector or the housing.  Such
captures will probably not be observable by the neutrino detector and
will artificially reduce the observed efficiency.  Secondly, we must
choose the source activity carefully so as to not produce an
artificially high measurement.  With high source activities comes an
associated \fixme{increased?} risk/probability of two or more neutron emissions awaiting
capture after a tag \fixme{clarify -- two emitted neutrons are 'tagged' but not 'captured'?}, artificially increasing the observed neutron
detection.  The best way to overcome this problem is to keep the source
activity low ($<$1000~Hz) while using simulations
to fully understand the effects of source geometry on efficiency.

Advantages:
\begin{enumerate}
\item Neutron-tagging source, neutron-detection
efficiency \fixme{measured?} on an event-by-event basis \fixme{clarify why this is an advantage}
\item Low event rate.  Deployment times will be lengthy \fixme{Time periods where source is in place? Why lengthy?}, leading to a smaller number of deployments overall. \fixme{not clear to me}
\item {Deployment locations essentially unlimited}
\end{enumerate}
	
Disadvantage:
\begin{enumerate}
\item  Slightly bulky due to scintillation crystal and source
containment; in addition, the containment may swallow up neutrons, reducing efficiency. \fixme{I reworded; check if meaning is right}
\end{enumerate}
	
\subsubsection{Californium (Cf)}

The Cf nucleus undergoes spontaneous
fission \fixme{true for 252 Cf only?}, simultaneously emitting prompt neutrons and gamma rays\fixme{both?} with
energies below 10~MeV.  The neutrons have a mean energy of 1.3~MeV and
a multiplicity distribution that is approximately Poissonian with a
mean of 3.787.   If a $^{252}$Cf source can be fully characterized
externally \fixme{i.e. calibrate the calibration source in a separate setup? What characteristic are you measuring if you know the multiplicity already?}, the detector neutron efficiency can be measured with just a
bare source \fixme{how does that follow?}, minimizing the associated hardware and reducing systematic
uncertainties.  Measurements of the neutron multiplicity within the
detector can then be compared with the known characteristics of the
source and with simulations.  Clearly, deployments at high activity would be
possible with such a source \fixme{Not clear to me! Is it because there's no extra hardware to capture neutrons?}, allowing quick measurements of the neutron-capture characteristics at many positions throughout the detector.

Advantages:
\begin{enumerate}
\item High rate \fixme{stated below, don't need twice: `many possible deployment locations'.} 
\item Short deployments \fixme{above, lengthy deployments were an advantage}, little dead time needed
\item Smallest and least bulky neutron source. 
\item Unlimited deployment locations.  
\item Small systematic uncertainties \fixme{did you talk about this?}.
\end{enumerate}

Disadvantage:
\begin{enumerate}
\item High energy e$^-$ and gamma-ray contamination of the
neutron-capture and prompt signal \fixme{not clarified in text}
\end{enumerate}

\subsubsection{Deuterium Tritium (DT)}
A DT generator has been employed at \superk{} for many years as an
energy-calibration source.  Fast neutrons emitted by the device create
a local pool of $^{16}$N in the detector via a $^{16}$O(n,p)$^{16}$N
reaction.  The subsequent $^{16}$N $\longrightarrow ^{16}$O + e$^{-}$ + $\nu_e$ emissions have a well-known energy distribution.  Relative to the low-energy (few MeV) LINAC \fixme{ref},
the DT generator has the advantage that it can be deployed at many
locations in the detector.

For neutron-detection efficiency measurements, the primary advantage
of this source will be the extremely high neutron flux.  The
$^{16}$O(n,p)$^{16}$N reaction above has a low efficiency, so most of
these neutrons are available for a neutron efficiency measurement \fixme{how does that follow?}.  It
also has a number of difficulties worth noting here.  First, the
hardware associated with the device is substantial, requiring a
particle accelerator, associated electronics and cables to be deployed
into the detector.  Issues such as shadowing due to the housing and
neutron loss within the hardware will have to be considered.  Secondly,
the associated $^{16}$N signal will be a
background.

Advantage:
\begin{enumerate}
	\item Huge number of neutrons
\end{enumerate}

Disadvantages
\begin{enumerate}
	\item Shadowing
	\item Neutrons lost in the hardware
	\item Bulky, and therefore limited number of deployment locations
	\item $^{16}$N contamination
\end{enumerate}

\subsubsection{Free Neutrons from Muon Spallation}

Free neutrons can result from muon spallation in the detector. 
Monitoring the position and time variations of the resulting neutron
captures will be a good test of detector (and gadolinium) stability.  
Such a test can reveal variations in Gd density over the entire
detector, free from deployment hardware and associated shadowing and
capture effects.  The absolute efficiency and position of the neutron
capture will not be measurable via this method.  However, variations
over time and position asymmetries will reveal themselves in the
data.  Additionally, the measurements will not impinge upon detector
livetime.   An example of the utility of this technique is the KamLAND
measurement of the fiducial-volume uncertainty \cite{Eguchi:2002dm}. %[1].

Advantages:
\begin{enumerate}
	\item No deployment hardware and therefore no loss of efficiency due
to shadowing effects or neutron loss in hardware.
	\item Events evenly spaced throughout detector volume.
\end{enumerate}

Disadvantage:
\begin{enumerate}
	\item Neutron capture location not known absolutely
\end{enumerate}


\subsection{Positioning and Space Requirements for Calibration}

Due to the potential for gadolinium-concentration variations from
place to place within the detector and over time, the same capability
for source placement will be required as for the energy calibration
(See \fixme{WBS 1.4.4.4}).   Wherever possible, access holes will be placed over
the deck at the top of the detector, allowing for a number of set
positions in $x$ and $y$.  The $z$ coordinate will be selectable with a
suitable cable/line length.  Obviously, the greatest possible number
and spacing of calibration ports over the deck will allow the greatest
possible $x$ and $y$ position freedom, however the placement of other
systems on the deck, such as electronics huts, cranes, cable trays, and so on,
will have to be planned in advance in consultation with the calibration
group.  Some sources (such as the DT generator) will require more room
around and above the calibration port.

\subsection{Safety Considerations}

The most important safety consideration of the gadolinium-monitoring
group will be the use of radioactive sources.  Like all federally
operated national laboratories in the U.S., DUSEL in South Dakota
will operate under a set of rules, procedures and controls for the
handling of radioactive materials.  It is each laboratory's
responsibility to oversee the handling of these materials on a
day-to-day basis.  The LBNE experiment, as a user of the facility, will
need to fulfill all the requirements of the DUSEL laboratory.

\subsubsection{DT-Generator Safety Considerations}

A DT generator is capable of releasing an enormous flux of fast
neutrons. The \superk DT generator system employs a simple sonic based
water detector attached to the cable above the unit.  A safety
interlock, which cuts power to the device until it is under water, must
be employed to guard against an accidental trigger.   Fully trained
calibration experts will be the only people permitted in the detector
dome during the DT calibration.  All personnel associated with the
deployment of this source will need to carry radiation monitors at all
times.

\subsubsection{Safety for Sealed Neutron Sources (Am-Be and $^{252}$Cf) :}

The DOE has defined a set of thresholds that apply to the
classification of radioactive sources.  In both cases (Am-Be and
$^{252}$Cf), a class III source should be sufficient for calibration
purposes.  Calibration workers, carrying radiation monitors, 
would be fully trained in the use of sealed sources.   All sources must
be protected with at least two independently leak-tested seals to
protect both the sources and the detector.  Assuming the height of the
vessel will be approximately 50 meters, the pressure at the base of
the tank will be six atmospheres.  All deployment containers will have to
be pressure tested to this level plus an as-yet-undefined safety
margin.


\fixme{Budget Description below Goes elsewhere!!}
%
Two possible tagged Am-Be sources will be considered.  Firstly one can
deploy a source in an optically clear container together with a
scintillating crystal.  Gamma-ray interactions in the crystal would
emit light isotropically, producing a tag signal in the detector PMTs. 
A related design may include a PMT with the crystal to register
gamma-ray interactions in the crystal directly.   In both cases the
source, PMT and crystal may be obtained commercially for approximately
\$6k.  A source container will have to be designed, built, pressure-tested and approved for this deployment, adding some uncertainty to the
cost.  Total estimate \$12k.

The $^{252}$Cf source will comprise only a source (\$3k) and another source
containment (\$6k).  Total \$9k.
%\end{indentation}

The DT generator system at \superk was built ten years ago for a total
of approximately \$120k to \$130k.  It consists of a commercial unit
worth about \$70k and auxiliary equipment, including a water proof and
pressure tested housing and water proof feedthroughs (\$50k to \$60k). 
Taking into account uncertainties such as shop labor, inflation, etc,
we estimate approximately \$200k for the LBNE system.

%Key Uncertainties

All of the proposed neutron-detection-efficiency calibration sources
have been used and deployed in past water Cherenkov experiments and
hence can serve as proof of concept.


==> volume-4-WCD/calib-install.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

\section{Calibration Installation (WBS 1.4.5.8)}
\label{sec:v4-calib-install}

\subsection{Requirements and Specifications}
\label{subsec:v4-calib-install-reqs-n-specs}

Blah blah on Calibration Installation Requirements and Specifications.

\subsection{Description}
\label{subsec:v4-calib-install-desc}

Blah blah on Calibration Installation Description.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../volume-4-WCD"
%%% End: 


==> volume-4-WCD/esh-approach.tex <==
%
% WCD/esh-approach.tex
%
\section{Approach}
\label{sec:v4-approach-esh}

The scientific goals of this experiment cannot be achieved without an effective safety and environmental protection program that is integrated into the overall management of the experiment. This presents some unique challenges since several laboratories and universities must interact with federal, state and local institutions. It is a goal of the WCD to comply with all applicable federal, state and local regulations. To accomplish this, integrated safety management is implemented to ensure that all stages of the project, planning, design and physical work are performed with attention to the potential hazards.

Work performed at collaborating institutions will follow the safety systems established at their location. Institutions in the collaboration that do not have a formal Integrated Safety Management System will, as a minimum, develop work plans that identify hazards and the means to mitigate those hazards. Work performed at DUSEL will follow the DUSEL Work Action Planning and Hazard Analysis procedure. Work cannot begin without a safety review or hazard analysis and approval. Formal procedures will be established where necessary to ensure that work is done safely and correctly. This is also an important aspect of the quality assurance (QA) program. 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../volume-4-WCD"
%%% End:


==> volume-4-WCD/esh-intro.tex <==
%
% WCD/esh-intro.tex
%
\section{Introduction}
\label{sec:v4-intro-esh}

The Long Baseline Neutrino Experiment (LBNE) proposes to perform
measurements of neutrino oscillations to test for violations of
CP-invariance in the lepton sector. Such a finding would have far
reaching impacts in particle physics, astrophysics and cosmology. The
experiment would also be in a unique position to investigate proton
decay with improved sensitivity, and to measure neutrino bursts from
supernovae.

To accomplish these goals, large Water Cherenkov Detectors (WCDs)
will be installed in new caverns at the Deep Underground Science and
Engineering Laboratory (DUSEL). Detection of events would be via large
arrays of photomultiplier tubes, as employed in previous
experiments. The neutrino sources would originate from accelerators
based at Fermi National Accelerator Laboratory (FNAL) and Brookhaven
National Laboratory (BNL). Upgrades to these accelerator facilities to
enhance neutrino production are being considered, but are outside the
scope of this document.

Personnel safety and protecting the environment are high priorities
for the Long Baseline Neutrino Experiment. The Hazard Analysis
Document is intended to identify those aspects of the experiment that
present potential hazards either to project personnel, the
environment, or the public at large. By determining the categories and
analyses used for those hazards, the document will show how each of
them can be mitigated. Many of the hazards that will be encountered
are of the types that have been encountered during past operation of
similar experiments. The construction of the facilities and
infrastructure both above and below ground are outside the scope of
this document. A Hazard Analysis Document (HAD) will address the
hazards associated with the assembly, installation, testing, and
operation of the experimental equipment. This document does not offer the level of detail that the
HAD will contain, rather it offers the strategy that will be employed
to identify and mitigate the hazards.



==> volume-4-WCD/integ-civil.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

\section{Civil Construction Interface (WBS 1.4.8.5)}
\label{sec:v4-integ-civil}

The Civil Construction Interface consists of management
oversight of engineering and designer effort to assist subsystems in
defining the experimental requirements as they pertain to space and
utility interface with civil construction of the facility. This includes
activity such as the definition of the cavern/vessel interface as
discussed in Section~\ref{sec:v4-water-contcavern_interface}. They will
interact with WCD subsystems and the WBS 1.6 Conventional Facilities group in defining
experiment to facility interfaces. They will incorporate as-built
facility documentation into 3D models of the WCD project 
complex as required for subsystems design and installation
planning.


==> volume-4-WCD/intro-physics.tex <==
\textbf{Neutrino beam oscillations}

The primary physics goal of LBNE is to measure the oscillations of
accelerator-generated neutrinos.  Oscillations occur due to the
quantum mechanical mixing between the flavor states of the neutrinos
($e$, $\mu$, $\tau$) and the mass states.  The mixing of three flavors
of neutrinos can be described by three mixing angles ($\theta_{12}$,
$\theta_{23}$ and $\theta_{13}$) and one CP-violating phase
($\delta_{CP}$).  The probability for neutrino oscillation also
depends on the difference in the squares of the masses, $\Delta
m^{2}_{ij} = m^2_i - m^2_j$; with three neutrinos, there are two
independent mass squared differences ($\Delta m^2_{21}$ and $\Delta
m^2_{32}$).  Oscillations of a muon neutrino beam over a long baseline
can be studied to measure $\theta_{23}$, $\theta_{13}$, $\delta_{CP}$ and
$\Delta m^2_{32}$.  In fact, all the neutrino oscillation parameters
can be studied in a large water \cherenkov detector, as $\theta_{12}$
and $\Delta m^{2}_{21}$ can be explored with solar neutrinos.

% \bf{$\nu_{\mu}$ disappearance}
The study of the disappearance of $\nu_{\mu}$ probes $\theta_{23}$ and $|\Delta
m^{2}_{32}|$.  Experiments suggest that $\theta_{23}$ is very close to
maximal ($\sin^{2}(2\theta_{23}) > 0.92$ at 90\% confidence
level).  One of the key questions LBNE will explore is whether
$\theta_{23}$ is significantly different from maximal.

% A study of $\nu_{\mu}$ disappearance requires selection of a sample of $\nu_{\mu}$
% interactions.  In a water \cherenkov detector, $\nu_{\mu}$ charged-current (CC)
% interactions, in which the $\nu_{\mu}$ interaction produces a charged
% muon, can be identified by a single characteristic muon ring.  The
% energy of a neutrino producing a single muon ring is reconstructed
% assuming the event was a charged-current quasi-elastic (CCQE)
% interaction, $\nu_{\mu} n \rightarrow \mu^{-} p$.  (The proton is typically below \cherenkov threshold.)  Given this
% assumption and the reconstructed energy and angle of the muon
% ($E_{\mu}, \theta_{\mu}$), the energy ($E_{\nu}$) of the neutrino is
% given by
% \begin{equation}
%  E_{\nu} = \frac{E_{\mu}m_{n} - \frac{1}{2}m_{\mu}^2}{m_{n} - E_{\mu} + p_{\mu}\cos\theta_{\mu}}
% \end{equation}
% where $m_{n}$ is the neutron mass and $m_{\mu}$ is the muon mass.
% 
% The main background to this channel are CC non-QE interactions, where additional particles are produced but not detected (due to reconstruction inefficiency or the threshold for \cherenkov emission).  The reconstructed energy using the above scheme for these background events will be lower than the true energy due to the missing particles.

% \textbf{$\nu_{e}$ appearance}
Observation of $\nu_{\mu} \rightarrow \nu_{e}$ oscillations are the
key to measuring $\theta_{13}$ and determining the mass hierarchy (the
sign of $\Delta m^{2}_{32}$, which can't be determined by $\nu_{\mu}$
disappearance).  The signature of CP violation is a difference in the probability for
$\nu_\mu \rightarrow \nu_{e}$ and
$\overline{ \nu_\mu} \rightarrow \overline{\nu_{e}}$ transitions.  The
signal for $\nu_{\mu} \rightarrow \nu_{e}$ oscillations is an excess of $\nu_{e}$-like interactions over the background expected from beam $\nu_{\mu}$ and $\nu_{e}$.
% In a water \cherenkov detector, the rings produced by
% muons have sharp edges, while those produced by electrons have fuzzy
% edges due to multiple scattering.  The signal for a $\nu_{e}$
% interaction is a single electron-like ring.  When selecting $\nu_{e}$
% candidate events, the backgrounds are primarily due to beam neutrinos,
% not cosmogenic or other sources.  It is easy to reject background due
% to $\nu_{\mu}$ charged-current (CC) interactions due to the
% distinctive muon ring pattern.  CC interactions from $\nu_{e}$ that
% are intrinsic to the beam form an irreducible background as the
% signature is exactly the same as the signal.  The other main
% background component is neutral-current (NC) events with a $\pi^{0}$.
% In NC events, a charged lepton is not produced, but other particles
% produced in the interaction can make \cherenkov light.  In particular,
% if a $\pi^{0}$ is produced, it can decay via
% $\pi^{0} \rightarrow \gamma \gamma$.  The $\gamma$'s form two fuzzy
% (electron-like) \cherenkov rings.  If the opening angle between the
% two gammas is small, the rings overlap and will sometimes be
% reconstructed as one electron-like ring.  In addition, if the decay is
% asymmetric, a small low energy ring might be missed.  In this way, the
% $\pi^{0}$ can generate an event topology that mimics the $\nu_{e}$
% signal.  The ability to reconstruct $\pi^{0}$'s depends in part on the
% density of PMTs.



\textbf{Astrophysical and extraterrestrial neutrinos}

A water \cherenkov detector at LBNE would have the potential to study
neutrinos from natural sources, for example:
\begin{itemize}
 \item Supernova neutrinos --- Studying the
 neutrinos emitted during a supernova could provide significant
 insight into these events.  A nearby supernova would produce a burst
 of neutrino events in a large water \cherenkov detector.  Nearby
 supernovae are rare (a few per century), and this is a strong
 motivation to maximize the live time of the detector and build
 multiple detector modules so that at least one module is always
 taking data.  There is a precedent for the detection of neutrinos
 from supernova bursts --- 19 events were seen in water \cherenkov
 detectors (IMB and \kamiokande) from supernova 1987a.  
\item Relic supernova neutrinos (also called the diffuse supernova neutrino
 background) --- Since nearby supernovae are rare, identifying the
 neutrinos from far away supernovae might provide the best chance to
 study them.  \superk has set the best limit on the flux of supernova
 relic neutrinos\cite{Malek:2002ns}, but the measurement is background limited.  Reducing
 background and lowering the energy threshold are key to observing these neutrinos.  The \superk limit is very close to theoretical predictions, shown in Figure~\ref{fig-srn-pred}\cite{Lunardini:2010ab}. The discovery of relic supernova neutrinos is within reach.
\item Solar neutrinos --- Study neutrino oscillations ($\theta_{12}$, $\Delta m^{2}_{21}$) and get a
 better understanding of the solar neutrino spectrum.  One important
 goal is the search for the as yet unobserved day/night asymmetry of
 solar neutrinos.
\item Atmospheric neutrinos --- Atmospheric neutrinos are unique among sources used to study oscillations: the oscillated flux contains neutrinos and antineutrinos of all flavors, matter effects may play a significant role, and the oscillation phenomenology plays out over several decades in energy and path length. These characteristics of the atmospheric flux make it an ideal source for studying a wide range of oscillation and mixing effects.

\end{itemize}

\begin{figure}
\begin{center}
 \includegraphics[width=0.8\textwidth]{volume-4-WCD/figures/SRN_predictions_fig}
 \caption{Comparison of \superk's upper limit on the flux of relic supernova neutrinos to a sample of theoretical predictions\cite{Lunardini:2010ab}.}
 \label{fig-srn-pred}
\end{center}
\end{figure}

\textbf{Nucleon decay}

One of the key predictions of Grand Unified Theories (GUTs) is a
finite nucleon lifetime.  The primary requirements for a proton decay search are mass
and livetime.  In addition, a low background rate and significant
detection efficiency are desirable.  There are two important modes that will be studied: $p \rightarrow e \pi^{0}$ and $p \rightarrow \nu K^{+}$.  These are the principle decay modes predicted by current models.

In a water \cherenkov detector, the signature for the $e \pi^{0}$
channel is 3 electron-like rings --- 1 from the electron and 2 from the
decay of the $\pi^{0}$ into two gammas.  The limit on this decay mode
set by \superk is $8.2 \times 10^{33}$ years at the 90\% confidence level\cite{2009gd}.
The detection efficiency for this mode is dominated by pion absorption
in the nucleus and cannot be significantly improved. An order of
magnitude improvement in this mode by \superk can only be achieved by
running \superk for an additional 30--40 more years.  The limit could be
pushed by a larger water \cherenkov detector at DUSEL.

The $\nu K^{+}$ channel is more difficult to observe in a water
\cherenkov detector, as neither of the final state particles are
visible --- the $K^{+}$ is produced with a momentum that is below the
\cherenkov threshold.  The kaon decays with a lifetime 12.4~ns by
$K^{+} \rightarrow \mu^{+} \nu_{\mu}$ or
$K^{+} \rightarrow \pi^{+} \pi^{0}$.  When a proton bound in an oxygen
atom decays, it produces a nitrogen ion in an excited state that
decays about a third of the time via a detectable photon of $\sim$6
MeV.  The signature of this decay in a water \cherenkov detector is
the delayed coincidence between the proton decay tagged by the 6~MeV photon
and the kaon decay.  Thus the energy threshold, which depends on the
photocathode coverage, must be low enough to detect the 6~MeV gamma.
\superk used this method to set a limit of $2.3 \times 10^{33}$ years\cite{Kobayashi:2005pe}.



==> volume-4-WCD/pmt-base-design-appx.tex <==
\begin{appendices}

\chapter{Design Considerations for the PMT Base} % RVB
\label{appx:pmt-base-design}

This appendix supplements the text in Chapter~\ref{ch:photon-det}, Section~\ref{sec:pmt-base-design}.

\section{Base Current and Power}

%standing current: curr in base w no light source
%base current: standing curr + curr effect from light

Whereas the PMT voltage ratios are determined, as described in
 Section~\ref{subsec:pmt-optoelec-char}, either
from the manufacturer's suggestion or from experimental optimization,
the current in the base (or the total resistance of the PMT divider
chain) is a separate parameter that must be optimized in its own
right. 

For a given PMT operating voltage, the power dissipated in the
base goes directly as the current ($P=I \times V$). That power needs to be generated,
regulated, delivered, and then eventually pulled out of the detector
as waste heat. Therefore it seems logical to reduce the power as much as
possible. However, we must take into account the relationship between base current (hence heat load) and signal current.

As the signal current increases and becomes a
larger proportion of the base standing current, the voltages across
the last few dynodes (the only dynodes with significant current draw)
are reduced as is the gain, and a non-linearity with rate (and
average pulse size) is introduced. Typically signal current is kept to about 1\% of the standing base current.

For the WCD, we expect most of the output current
to be dark current---well under 10~kHz of single PE. At a nominal gain of $10^7$,
this yields a (dark) signal current of only $1.6 \times 10^{-8}$~A. With a standing base current two orders of magnitude higher ($10^{-6}$~A), and very high resistances (outside the normal value range \fixme{of what values?}), the heat load would
only be 2~mW/PMT (i.e., an insignificant 100~W for a detector of 50,000
PMTs).

We plan to push the standing base current higher
by one or two orders of magnitude to greatly increase the linear range
for unusual events (e.g., a supernova) at a very modest
increase in overall system power consumption. 

To avoid a gain droop in the event
of a short series of very large pulses, we can place storage capacitances across the last few dynode stages to store enough charge between pulses to avoid distorting the dynode voltage ratios. For a nominal 100~V drop between the last two dynodes, a 1~nF capacitor across them would support the base current with only a $\sim$2\% drop in voltage.

% Not sure this example is needed. ...  For example, a cosmic-ray shower that produces ten different muons passing through the detector in 1~$\mu$sec with an average of 100~single PE per PMT per muon would represent a peak current for that microsecond of 1.6~mA at the last dynode of each PMT. For a 1~$\mu$A or even a 100~$\mu$A base current this would totally shut down the PMT. However,  

We will need to determine the actual size of these local decoupling
capacitors by examining a range of possible
interesting physics cases, but the 1~nF in this example is a reasonable
and plausible size to start with. Capacitors rated at 200~V in the pico to a few 
nanofarad range are widely available in moderate-size packages.

\section{Signal Cable Termination}

The long signal cable from the PMT base to the electronics is a transmission
line that will be terminated at the electronics end. It is described in more detail in Section~\ref{sec:v4-photon-det-cable-assy} and Section~\ref{sec:v4-elec-readout-design-char}.  
Because that termination will not be a perfect impedance match for the cable --- typical mismatches
are on the order of 1 or 2\%---some reflection back to the base will occur. If the base is not back-terminated then
large PMT pulses will produce very late reflections back at the
electronics. Back-termination of a similar 1--2\% accuracy will reduce
the resultant reflection to roughly $10^{-4}$ such
that only extremely large pulses, far beyond the expected dynamic
range of the system, could produce single-PE-sized reflections. The
back-termination, of course, must be capacitively coupled to avoid
shorting out the HV supply; this implies a termination resistor
and a capacitor capable of withstanding the full PMT operating
voltage.  The use of a capacitive back-termination does, however,
imply that the far end of the cable, the electronics end, must match
the complex impedance at the base. Figure~\ref{fig:capmismatch} shows
the effect of badly mismatched capacitive coupling at the
electronics. This emphasizes the need for careful co-design of the PMT
base and the front-end electronics.

\begin{figure}[ht]
\begin{center}
\begin{tabular}{cc}
\includegraphics[width=0.50\textwidth]{volume-4-WCD/figures/CableTerm3Sch.pdf} &
\includegraphics[width=0.45\textwidth]{volume-4-WCD/figures/CableTerm3wave.pdf} \\
(a)Schematic & (b) Pulse simulation 
\end{tabular}
\end{center}
\caption[Simulation of the effect of mismatching the front and back terminations on the PMT base.]
{Simulation of the effect of mismatching the front and back terminations on the PMT base.
The three different cases are (left), top to bottom, schematics, matched capacitances, 
much larger at the preamp, much smaller at the preamp. 
The waveforms (right) are arranged in the same order left to right.}
\label{fig:capmismatch}
\end{figure} 

\section{Damping Resistors to ??}

In addition to the energy-storage capacitors across the last few
dynodes, it is often useful to provide damping resistors in series
with each of the last few dynodes. This damping is needed because of
the relatively large currents and fast rise times associated with the
large pulses on these dynodes and the inherent inductive nature of the
connection to the dynode --- a long conductor reaching into the dynode
assembly. \fixme{you don't say exactly how the damping resistors work, or what they do. I assume they limit the current so that the induction is reduced... but it seems they'd change the voltage drop. Please clarify.}
These damping resistors need to be determined experimentally
for the particular PMT selected as the actual inductance depends upon
the mechanical design of the internal structure. The damping resistors
are typically in the range of tens to hundreds of Ohms.

\section{Achieving High Reliability}

In order to build a reliable device, there are several areas to
consider. The components used (resistors, capacitors, and diodes)
must, of course, be highly reliable in and of themselves and the
handling of those components during the assembly process must satisfy
the component manufacturer's requirements. But modern, high-quality,
commercial electronic components are both extremely reliable and the
handling protocols are well described. The more challenging issue is
the physical design of the printed circuit board and its connections
to the PMT and the cable since the voltages involved are relatively
high --- into the regime where significant care must be exercised. The
high-reliability requirement basically implies that the design needs to
be quite conservative in terms of voltage stress --- this in turn implies
keeping traces or pads at very different
voltages distant from each other, making sure that there is sufficient dielectric material (e.g., board thickness)
between traces at widely separated voltages,
and avoiding the sharp corners or other features that might encourage
corona discharge.

\section{Radioactivity of Base Components}

The last area of concern is the total radioactivity burden imposed by
the base components. As the PMT base is situated near the
photosensitive surface of the PMT, radioactive decays in the base can
cause unwanted photoelectrons in the PMT --- either through Cherenkov
light in the PMT glass, or gamma or beta interactions that make light
in the surrounding water. The as-yet-unknown requirement on total
radioactivity in the base {\em may} affect the choice of construction
materials. For instance, ceramic capacitors and flame-retardant circuit
board materials both tend to have relatively high concentrations of Rn
and Th, and it may be necessary to go to film capacitors
and/or Kapton printed circuits.
\end{appendices}



==> volume-4-WCD/pmt-charact.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.


\subsection{Optimization and Characterization Program}
\label{subsec:v4-photon-det-pmt-opt}
 
Due to the central role of the PMTs in the WCD and to the potential mechanical risks they present, we have begun implementing a comprehensive program to ensure that the PMTs and the PMT assemblies (PAs, described in Section~\ref{sec:v4-photon-det-pa}) can withstand the experimental environment for the expected \lifetime lifetime. We will test optical/electrical properties, too, but will focus on mechanical robustness, since that is the area of particular concern.
%Much of the program extends beyond the PMT to its assembly , including any light-enhancement additions. 
The program consists of several phases that overlap in some cases.
\begin{itemize}
\item Evaluation:  a near-term project begun in early 2010 that will extend roughly through 2012, ending with the selection of the model. The goal is to determine the best available model in terms of performance, cost and vendor capability and reliability.
\item Optimization: a project that overlaps the latter part of the evaluation phase and continues into the procurement period. The goal is to work with potential vendors to optimize the PMT model for LBNE both in terms of performance and cost. In this phase, measurements of the effects of variations in response as a function of gain and high voltage, for example, will provide us with the best set of PMT operational parameters. \fixme{Check:} We will also aim to optimize the glass envelope and other mechanical features to prevent against implosion.
\item Characterization: a long-term project in which we will
  rigorously test the selected model's optical, electric and
  mechanical properties to gain a deep and broad understanding of its
  behavior along with any associated light-enhancement assembly or
  mechanical support. The knowledge gained in this phase will be fed
  into simulations that we will use to predict the PMT behavior under
  actual experimental conditions. This phase overlaps the latter part
  of the optimization phase and continues throughout the PMT
  production period and past the Project phase of LBNE.
\end{itemize}

%We describe these phases further in Appendix~\ref{appx:pmt-char}. %filename pmt-mech-char-appx; maybe shouldn't have 'mech' in title

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%	Measurements of the PMT optical and electronic
%characteristics play three central roles for the WCD. 
%\begin{itemize}
%\item They will inform the selection of the PMT type for the
%experiment. The experiment's physics program is likely to be enhanced by the
%PMT type that has the best timing or charge response, higher efficiency at the
%wavelengths expected to arrive at the phototube array through the transfer
%function of the water or possible intervening mechanical shield, or lower dark
%current. We refer to this phase of measurements the `PMT evaluation phase' and
%it will primarily be funded through the NSF S4 grant.  

%\item The
%benchtop PMT measurements will help optimize the PMT and
%base circuitry.  Measurements of the effects of variations of response as a
%function of gain and high voltage, for example, will provide us with the best
%set of PMT operational parameters.  

%\item Lastly, a full characterization of the PMT,
%including all relevant optical parameters for the PMT itself and any associated
%light-enhancement assembly or mechanical support, will allow us to model the
%phototube detection process in great detail, thus minimizing systematic
%uncertainties in the full detector.
%\end{itemize}



==> volume-4-WCD/pmt-design.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

\subsection{Design Considerations and Reference Design}
\label{subsec:v4-photon-det-pmt-design}

\fixme{This info may change over the next several months. Anne 12/15/10}

We chose the high-quantum-efficiency (HQE) Hamamatsu 10-in R7081HQE PMT for the reference design. Considerations that went into the choice include:
\begin{itemize}
\item The R7081HQE is an off-the-shelf item, and therefore schedule and cost
risks are minimized.
\item Initial testing has demonstrated that this PMT is relatively resistant to the high pressures in the WCD. %(as compared to a larger PMT, e.g., 12~in). New info coming in may not jive with this comparison 12/15/10

\item The R7081HQE has been used by other experiments such as ICECUBE and
many LBNE collaborators have experience with the device.
\item The high quantum efficiency of the PMTs allows fewer channels and thus leads to cost savings on electronics and cabling.
\item In our own benchtop
tests, the R7081HQE has been shown to meet our requirements, as outlined in
Section~\ref{subsec:v4-photon-det-pmt-reqs-n-specs}. 
\end{itemize}

We are examining two other potential PMTs as alternatives, an HQE 12-in PMT from Hamamatsu, and an 11-
in PMT made by ETL.  These PMTs will be subject to the same evaluation
process as the reference design model and we will choose based on an optimization of cost and weighted risks. If other competitive PMT models are developed in the short term 
%---e.g.,a high-quantum-efficiency version of the Hamamatsu 12-in PMT---
we will also evaluate it (them).


==> volume-4-WCD/pmt-mech-char-appx.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

\begin{appendices}
\chapter{PMT Characterization Appendix}
\label{appx:pmt-char}

As we stated in Section~\ref{subsec:v4-photon-det-pmt-opt},  we have begun implementing a comprehensive PMT and PA characterization program. The program consists of three phases: Evaluation, Performance Optimization and Characterization.

\section{PMT Evaluation}

The PMT evaluation phase is a near-term project that will extend
through roughly the end of 2012. 
During this phase, the parameters discussed in Section~\ref{subsec:v4-photon-det-pmt-reqs-n-specs}
will each be measured, and compared to the requirements for
LBNE physics.  These parameters will be measured both with Cherenkov
sources at single-PE levels, as well as with fast LEDs or lasers
to help determine dynamic range and linearity.  The effects of
magnetic-field compensation on PMT efficiency and timing will also be
determined, to help decide how much compensation the full detector
will need.  Figure~\ref{fig:pmttim} shows a time-residual curve
for a Hamamatsu R7081 10-in high-quantum-efficiency (HQE) PMT, and
Figure~\ref{fig:pmtq} shows the charge spectrum for the same PMT, both
measured with single photon illumination from a Cherenkov
source. 
\begin{figure}[htb]
\begin{center}
\includegraphics[height=0.4\textheight]{volume-4-WCD/figures/r7081hqe_time}
\caption{Time residuals for R7081HQE PMT.  \label{fig:pmttim}}
\end{center}
\end{figure}
\begin{figure}[htb]
\begin{center}
\includegraphics[height=0.4\textheight]{volume-4-WCD/figures/r7081hqe_charge}
\caption{Charge spectrum for R7081HQE PMT.  \label{fig:pmtq}}
\end{center}
\end{figure}

	During the evaluation phase, we will examine several of the robustness criteria
discussed in previous sections, such as the
PMT's behavior after high illumination (and any resultant permanent
damage). We will also search for any spurious light emission from the PMTs,
effects from temperature excursions or seismic vibrations. These studies will have
implications for PMT storage and safe handling.  

	The evaluation phase will include some stability issues, for example
determining gain stability over the given period of weeks or months, to ensure that
the selected PMT will not require
calibrations too frequently.

	The majority of the budget for these tasks comes from the NSF S4 grant,
from ARRA funds, and from institutional contributions (start-up packages or
already existing equipment). 

\section{PMT Performance Optimization}

	The optimization program will begin during the evaluation phase, but
likely last into the early parts of the subsequent characterization phase.  The
program includes tasks intended to determine the effects of the
light-enhancement assembly, the required magnetic field compensation, and the
PMT gain and voltage distribution.  The tasks will include
measurements of PMT photon-detection efficiency as a function of position and
angle across the photocathode face, for Cherenkov light in water (and air).
These measurement will determine the relative effective
efficiency of different PMT candidate models and inform the
design of possible light-enhancement assemblies.  Studies of the PMT timing and
efficiency as a function of magnetic-field compensation will 
determine how much the Earth's field will need to be cancelled underground
in the detector volume.  

	The operating gain of the PMT will also need to be optimized, to ensure clean observation of
 signal pulses above noise after the cable dispersion and
attenuation, to determine whether the PMT timing can be narrowed with higher
voltages, and to ensure that dark current remains at reasonable levels.  A
further optimization of the voltage distribution across the PMT dynodes may
involve fixing the cathode-to-first dynode voltage for all PMT gains.  This
fixed voltage may improve both the peak/valley ratio for individual PMTs
(because the voltage can be made higher without raising gain or causing the 
dark current to become too high) and also reduce PMT-to-PMT variations in
charge and timing resolution.  The effects of these different
voltage-distribution schemes on other phenomena such as latepulsing and PMT
`flashing' will be studied during this phase. 

	A further optimization task during this time will be the determination
of cable-transmission characteristics that will help minimize signal loss.  In
addition, cable compensation schemes may be investigated to remove the
dispersion in the PMT signals in order to obtain better timing and charge
resolution after the signals pass through the long cables.


\subsection{Optical and Electronic Characterization}
\label{subsec:v4-photon-det-pmt-opt}

	Measurements of the PMT optical and electronic
characteristics play three central roles for the WCD. 
\begin{itemize}
\item They will inform the selection of the PMT type for the
experiment. The experiment's physics program is likely to be enhanced by the
PMT type that has the best timing or charge response, higher efficiency at the
wavelengths expected to arrive at the phototube array through the transfer
function of the water or possible intervening mechanical shield, or lower dark
current. We refer to this phase of measurements the `PMT evaluation phase' and
it will primarily be funded through the NSF S4 grant.  

\item The
benchtop PMT measurements will help optimize the PMT and
base circuitry.  Measurements of the effects of variations of response as a
function of gain and high voltage, for example, will provide us with the best
set of PMT operational parameters.  

\item Lastly, a full characterization of the PMT,
including all relevant optical parameters for the PMT itself and any associated
light-enhancement assembly or mechanical support, will allow us to model the
phototube detection process in great detail, thus minimizing systematic
uncertainties in the full detector.
\end{itemize}

\section{PMT Optical Characterization}

	The longest-term program will be the full characterization of the PMT
and its assembly, including any light-enhancement addition.  Our goal is a
complete optical model for the PMTs that can
be used in the Monte Carlo simulation of the detector.  Previous experiments,
including SNO and Auger,
have been able to measure and model not only the properties of the PMT glass,
but the complex index of refraction of the photocathode material and optical
properties behind it, such as the reflectivity of the dynode stack.  This
has the advantage that it provides a physical model for all incident
wavelengths and angles of light.  Correlations between photon timing from PMT
reflections and PMT inefficiencies are naturally taken into account.
Ultimately, such modelling reduces systematic uncertainties on the detector, by
correctly predicting the energy response and vertex accuracy of the detector as
a function of position within the detector.

This PMT characterization program will require several light sources of
different wavelengths and different incident angles, on many PMT
samples.  It will need to be done across many PMT batches, as optical
properties have been known to vary during the manufacturing process
(sometimes intentionally).  The optical parameters will be used to
build a full PMT model that can then make predictions for Cherenkov
sources and be tested against those sources to see the degree of
agreement.

	In addition to the optical model, the final timing and charge model,
with the fully optimized PMT will be done during this time and added to
the simulation.  The end result will be a complete PMT model that can be used
in simulations up until the time the detector begins to take data. At that
point, in-situ measurements will either confirm the ex-situ model or replace
it, based upon the calibration suite discussed in Chapter~\ref{sec:v4-calib-introduction}
of this volume.


%%%%%%%%%%%%%%%%%%

\section{PMT Mechanical Characterization}

\fixme{There's text I need to put here}

\subsection{Photo-multiplier Pressure Performance} 

The static pressure  performance of the PMT will depend on 
the stress level in the glass shell, whether the 
glass is in compression or tension, the surface characteristics of
the glass bulb including damage due to abrasion and handling, 
and finally the stress induced corrosion of the glass bulb over the 
lifetime of the experiment.   

\underline{\bf Qualification of the glass } 

The typical glass used for the PMT bulbs is called borosilicate glass which 
has about 70\% $\rm SiO_2$ and 20\% $\rm B_2 O_3$, with rest made of 
various metal oxides.  An industry standard borosilicate glass is 
considered Schott 8246 which was used by the SNO collaboration. 
The exact chemical makeup of the glass varies  for different 
suppliers of the glass. A single PMT vendor may use several glass suppliers. 
Moreover the properties of the glass depend on the annealing temperature 
and the cooling conditions used during the bulb making process. 

Theoretical strength of glass \fixme{refer to Glass Science} 
is known to be as much as 20~Gpa. But in normal circumstances 
glass strength falls short by as much a 3 orders of magnitude. 
As an example, the glass bulbs for Hamamatsu R7081 are 12~cm in 
radius and 3~mm thick. If we make the 
assumption of a spherical bulb, 
at the bottom of the detector with  5.8~bar of 
static pressure the stress level in the glass will be 

$$S = {P r\over 2 t} \approx 12 {\rm Mpa} $$ 

where $P$ is the static pressure, $r$ is the radius and $t$ is the thickness.
This stress level is only a factor of 2 below the breaking point of ordinary glass. 
The actual shape of the bulb will raise the stress level by about a factor of 
2 in the neck of the PMT bulb if the thickness is the same for the entire 
glass envelope.  


Considering that we intend to purchase approximately 100~tons of glass in the form 
of PMTs, and this is perhaps the most crucial components of the 
detector, we will carry out the following program of activities: 
\begin{enumerate} 

\item We have sought glass expertise from the Inamori school of engineering 
at Alfred university in New York. Specifically the glass experts at Alfred 
will test the glass supplied by our vendors and qualify it as suitable for 
our detector. An initial report based on measurements with rods made of 
supplied glass is in preparation for CD1. 


\item There will be interaction with the PMT vendors specifically concerning the 
glass and requirements on the mechanical and chemical aspects of the glass will be 
created in collaboration with Alfred. 

\item  Specifications on the handling of the PMTs will be created 
for both transport and storage since it is clear that surface damage to 
the glass can have dramatic impact of its pressure performance. 


\end{enumerate} 



\underline{\bf Bulb performance} 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.70\textwidth]{volume-4-WCD/figures/pmt-press-test}  
\end{center}
\caption[Pressure history of several PMT's tested in a pressure vessel at BNL. ]
{Pressure history of several PMT's tested in a pressure vessel at BNL. 
The solid lines are for mechanical samples of R7081 tubes. The black dashed 
lines are for 2 EMI 9354 8~inch tubes, 
the orange dotted lines are for 2 Photonis XP1807 12~inch. The failure modes for 
these three types of tubes are explained in the text. }
\label{pmt-press-test}
\end{figure}  


Pressure performance of the PMT bulbs will be tested in a dedicated
pressure vessel at BNL. The pressure vessel is instrumented with 
both static and dynamic pressure sensors as well as a fast motion 
camera.  Several initial tests were conducted with a few samples of 
PMTs from three vendors. The pressure was raised hydrostatically 
in small increments until the bulb imploded (See Figure~\ref{pmt-press-test}. 
  The video of the breakage 
and photographs of the remaining shards were  used to understand the mode 
of failure. 

These tests were carried out with bare bulbs without a water proof base. 
Failure mode for the Hamamatsu R7081 was at the bottom of the bulb for all 6 tests. 
After failure the dynode structure was observed to move within 4~ms to the top of the 
bulb and penetrate the dome, thus causing a second break in the bulb. Water was observed 
to in-rush first through the bottom of the bulb and second through the top.  

The bulb breaks for the other PMT types were not with sufficient statistics, but they 
were observed to break slightly below the dome at the place were the dome 
curves into the neck. This is the location of maximum stress. Furthermore, the EMI 9354 
tubes tested were known to be built with thinner glass and were not meant for 
high pressure applications.  

With these initial tests we have understood the basic parameters of a PMT implosion: the 
static pressure, the time scale of implosion, the instrumentation needed to measure 
the implosion, etc.  We have also understood that the pressure rating supplied by Hamamatsu 
on the R7081 of 0.7~Mpa is essentially correct since of the 6 tests
 no R7081 tube imploded below 1.0~Mpa.  Several more tubes were cycled upto 
0.85~Mpa several times
with no failure.  

The BNL facility will now be used for higher statistics long term testing.  
Pressure control instrumentation is in development to allow variable 
loading rates for testing. 


\underline{\bf Time to failure for glass tubes} 


The PMTs will be submerged under ultra pure water 
upto a depth corresponding to $\sim$ 5.8 bars
of pressure for $\sim$20 yrs. It is well known in the glass material sciences that 
glass can undergo stress induced corrosion. Detailed models for 
this corrosion vary, however the main
mechanism is thought to be due to small surface cracks in glass. 
The cracks act as concentrators of stress. When they become sufficiently deep due to 
corrosion  the 
concentrated stress will eventually exceed the strength of glass.  
Stress induced corrosion will eventually lead to failure. 

We intend to have a step-by-step program of measurements that will lead to a 
statistical understanding of the probability of failure under static load over 
a long period of time.    

{\bf We require that the probability of failure as a function of time does not 
grow slowly with time. In such a condition, the time to failure becomes 
highly uncertain. If there are to be failures we prefer that they begin 
rapidly after a fixed period of time.} 

The measurement of the time to failure curve cannot be performed by measurements
over very long periods of time. Instead, our Alfred colleagues have suggested
that we perform measurement of the pressure at failure (PAF) as a function of the 
rate at which the pressure is applied (loading rate).   The PAF is expected to 
be lower at smaller loading rates.   Ideally we prefer to have 
glass that has no dependence on the loading rate.  We will therefore obtain a sufficiently 
large samples of bulbs and perform  measurements of PAF under different loading rates.  
The model of crack formation and propagation allows us to relate the measured curve to 
the time to failure.  The method of Wiebull statistics will be employed to use the 
statistically limited data. 
An illustration of static and dynamic fatigue curves is 
in Fig. \ref{fatigue}.

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/static-fatigue}
\includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/dynamic-fatigue}  
\end{center}
\caption[Fatigue curves of glass.]
{Fatigue curves of glass.  The static fatigue curve is shown on the left. The horizontal scale is 
for illustration only. For long times the stress at failure becomes less and less
certain.  The dynamic fatigue curve for various conditions is shown on the 
right. Conditions in which there is a substantial dependence (high slope) are 
not desirable, since they will lead to poor static fatigue limits.}
\label{fatigue}
\end{figure}  


\underline{\bf Decision on pressure housings} 


If the dynamic fatigue tests combined with the analysis of glass
indicate that there is substantial probability of PMT failures before 
a 20 yr lifetime, we will deploy pressure housings on the PMT bulbs.
In this case, the PMT bulbs will no longer be in contact with the 
ultra pure water.  

It is at this time uncertain if we will deploy the pressure housings for 
only the lower part of the detector or if they will be used for the entire 
detector. The effect of the pressure housings on the optical performance 
must also be understood. 


\underline{\bf Quality assurance plan during production} 


The time to failure data will be continuously improved during the 
PMT production period. We anticipate that we will obtain mechanical 
samples of bulbs during production. These bulbs could be bulbs that 
have failed the electrical tests.  It is at this time unclear 
how many such bulbs will be available. 
We are planning to utilize these mechanical samples corresponding to 
1\% of all production for destructive testing at various loading rates. 
At present time, this sampling rate corresponds to approximately 100 to 300 
bulbs per year as the production proceeds.  


\begin{enumerate} 

\item The mechanical samples will be obtained uniformly during the production 
period.  

\item We will require that these samples correspond exactly to the 
final product in mechanical detail, but may have failed electrical tests.  

\item The BNL pressure tank or another similar pressure tank will be moved to 
the final production facility for these PMTs. Dedicated technical staff 
will test each of the mechanical samples at different loading rates. 

\item The data will be combined to obtain a high statistics 
dynamic fatigue curve.  

\item The testing will also determine uniformity of performance during 
the entire production period. If there is significant deviation in 
the performance of the bulbs  there will be feedback to the vendor. 
 

\end{enumerate} 



\section{Chain reaction mitigation} 

\underline{\bf Description of problem} 


As we have remarked above 
the implosion of a 10-12 inch glass bulbs will take place over a 
$\sim$4 ms period. 
During this period water will rush inwards through the breakage in the glass.
At the end of this period the water velocity will come to an abrupt halt and 
the kinetic energy of the water will be transformed into a shock wave 
propagating outwards.  

The shock wave is characterized by the time at which the shock wave starts 
after the beginning of the collapse,  the peak pressure in the shock wave,
the width of the shock wave. The total impact energy in  the shock wave is 
an integral over the shock wave width, and it will fall as $1/L^2$ where L is the 
distance from the tube.  


A back of the envelope calculation of the peak pressure 
in the shock wave can be performed using some simplifications. We assume 
that it is an isothermal process, and about half of the released energy is converted 
to compressive energy. Using the bulk modulus of water of $M=2.2\times 10^9$Pa, we 
obtain the following by dimensional analysis:

$$P^2_{peak} = {2\times M\times P_{static}\times V_{tube}\over V_{pulse}}$$

Here $P_{peak}$ is the peak pressure, $P_{static}$ is the static load, 
$V_{tube}$ is the volume of the PMT, and $V_{pulse}$ is the volume of the pressure 
pulse as it passes the neighboring PMT. 
We assume the pressure pulse volume to be $4\Pi L^2 \times r$, where $r$ is the 
radius of the tube.  For $L=0.5 m$, $r=0.125 m$, $P_{static}=5.8 bar$, the peak 
pressure is calculated to be $\sim 7$Mpa.  This is an overestimate of the peak 
pressure because the approximation does not take several things into account. In 
particular, the speed of the implosion process, in which the glass might break 
at various places differently, has a big effect on the timescale of the process. 
Nevertheless, the formula shows two interesting effects: the peak pressure 
appears to rise as the square root of the static pressure, and the 
peak pressure drops as $1/L$ from the phototube.  The actual situation 
will be more complex, but the lesson from the simple analysis is that 
the scaling with static load and distance will not be linear or as $1/L^2$,
 respectively. 


To understand the full history of the shock wave, a more detailed analysis is needed.
Such an analysis can be found in reference~\cite{Turner2007}.
The result of this analysis is displayed in Figure~\ref{shock} and Table~\ref{shktab}.
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/pmt-press-pulse}
\end{center}
\caption[Two dimensional simulation of the time history of a bulb implosion. ]
{Two dimensional simulation of the time history of a bulb implosion.  Simulation 
is by Steve Turner from NUWC.}
\label{shock}
\end{figure}  
The analysis was carried out with special hydrodynamic code run in two dimensions.
The pressure history shown in the figure is at 15 cm from the center of the bulb. 
The peak value at 50 cm will be at least a  factor of 3.3 times smaller. 
Computational prediction of an implosion pressure pulse needs to include the failure
time history of the structure; otherwise it will over-predict the pressure time history.
This is shown in Table~\ref{shktab}. 
\begin{table}
\begin{tabular}{c|c|c|c}
Case & Collapse Time & Peak Pressure & Impulse \\
\hline 
   &   {ms}   & (MPa)  & (Pa-sec)  \\
\hline 
Spherical gas bubble & 4.3 &  13.8 & 2.05 \\
\hline 
Spherical gas bubble &  4.5 & 10.3 & 1.95 \\
with glass layer    &   &  &  \\ 
\hline  
PMT shaped gas &  4.3 & 22.2 & 1.67 \\
bubble       &     &   &  \\
\hline  
PMT shaped gas   &   5.3 & 12.7 & 1.50 \\
bubble with glass  &    &   &  \\
layer and 250m/s   &    &    &  \\
glass failure rate &   &   &  \\
\hline  
\end{tabular} 
\caption[Summary of PMT implosion analysis.]
{Summary of PMT implosion analysis.
The PMT bulb was assumed to be a 10 inch bulb. The PMT 
shape was assumed to be similar to the Hamamatsu R7081 
tube.  
 The  peak pressure  was recorded at 15 cm from the center of the
bulb.  
Analysis  by Steve Turner.
\label{shktab}
}
\end{table}
A PMT shaped glass bulb was simulated by first assuming 
that the entire glass envelope disappears and then assuming that the glass disappears in segments 
at a speed around the first breakage point (assumed to be at the neck) at a rate of 
250 m/sec.  In the second case, the implosion peak pressure is considerably smaller, although
the impulse, defined to be the integral of the pressure in time, is not much smaller. 
Although the implosion mechanism and the effects of the surrounding structure can be quite complex, 
the single parameter, the speed of glass failure, can be used to model the data at least to 
first order.  It also gives us the basic understanding needed to prevent a chain reaction.
We will have to devise structures and/or  protection mechanisms that slow down the in-flow of water 
in case of a PMT failure. By elongating the time scale, we will be able to lower the 
peak pressure in the shock wave.  


\underline{\bf Comparison to previous experience} 

There are two previous experiments at sufficiently large scale to 
provide us valuable experience.  The SNO experiment had 
9438 inward facing and 91 outward facing 
 PMTs (8 inch diameter Hamamatsu R1408, average glass thickness $\sim$2 mm) made from Schott 8246 glass 
(\fixme{refer to SNO NIM paper}. These tubes were placed in ultra pure water 
at depths ranging from 0.6 bar to 2.15 bar.   The tubes were housed in an ABS plastic 
 holder, which also formed a light-concentrator. In approximately 8 yrs of operation,
SNO did not experience any PMT implosions and no chain reaction events. 

The second example is \superk in which there are approximately 
11,000 PMTs (20 inch diameter Hamamatsu R3600, average glass thickness $\sim$ 4 mm) 
and $\sim$1900 outward facing 
PMTs (Hamamatsu R1408) most of which were recycled from the IMB experiment. 
The tubes are in ultra pure water at a maximum pressure of 3.8 bar. There are 
$\sim$ 1800 tubes at the bottom experiencing maximum pressure. 
The \superk detector ran from 1996 to 2001 (4.6 yrs) with high efficiency
and no failures. In November 2001, during refilling operation after some repairs,
an apparent cascade of implosions triggered by a single PMT implosion (at 3 bars of pressure) 
destroyed 
more than half the PMTs in the detector. Since that event the detector was refitted 
twice: once by redistributing the remaining tubes and later by rebuilding 
the entire detector. In the post chain reaction phase, the PMTs were covered 
by an acrylic shell that slowed down the in-flow of water to prevent chain reactions. 
The \superk collaboration has kindly offered documentation and 
expertise gained due to this unfortunate accident. 

In brief, the conclusion of the analysis of the \superk event is
as follows: 
The single PMT that triggered the chain reaction was most likely damaged 
due to impact during the upgrade work at the neck. Computer modeling 
indicated that a shock wave was generated 10 ms later (due to the 
large size of the SuperK tubes the time scale for implosion is longer),
the peak pressure on adjacent tubes was more than 10 MPa with width of 50 $\mu$second.
Finally, testing showed that the shock wave itself was responsible for failures in 
adjacent tubes: it was not movement of the PMTs or other collisions. 

\superk has been rebuilt to have the entire number of phototubes, except for the 
acrylic shells on each tube,  and has been running since 2006 with no  PMT implosions.  
Table~\ref{tabstress} compares the SNO and \superk experience with the water 
Cherenkov counter for LBNE. 
\begin{table} 
\begin{tabular}{l|c||c|c|}
       &  LBNE &   SNO & SuperK \\
\hline 
Tube &  10-12 inch & Ham-R1408 & Ham-R3600 \\
Dia (cm) &  25-30 cm & 20 cm & 50 cm  \\ 
Thickness (mm) & 3-4 mm & 2 mm & 4 mm \\ 
Pressure (kPa) & 580 & 215 & 380 \\ 
Stress (Mpa) & 12 & 5.3 & 12 \\ 
Number & $\sim$50000 & $\sim$9500 & $\sim$ 11000 \\
lifetime (yrs)  &  20 & 10 & 5 \\ 
\hline 
\end{tabular} 
\caption{Comparison of LBNE parameters with those achieved in SNO and SuperK.} 
\label{tabstress}
\end{table} 
We use the simple stress formula for a spherical bulb to 
compare the stress level experienced in the glass.  The table shows that in fact 
the stress performance achieved in SuperK is similar to what is needed for LBNE.  


\underline{\bf Description of Propulsion Noise Test Facility} 

Early in the design process we found it essential to have a means of 
testing the entire PIU structure including PMTs to make sure it is 
resistance against the type of implosion chain reaction that 
superk suffered.    The testing apparatus must be on a proper scale.
The pressure vessel at BNL was found to be inadequate for this task 
because it is too small compared to the size of the PMT itself. 
In the small BNL vessel ($\sim$ 400 liters), after a 5 liter  PMT implodes 
the pressure is  completely relieved because of the change in 
volume. This does not allow a shock wave to develop in the same manner 
as the real detector. The second requirement on such a facility was that it 
must be large enough to allow measurement of the implosion and its aftermath 
for at least 10 ms without any acoustical  reflections from the walls. 

There are only two ways to perform such testing: testing in open water 
from a ship or a platform or a large pressured tank.   Initial estimates
for open water testing had to include the costs for ship or platform 
rental. These can range between \$25,000 to \$50,000  per day. In addition,
the clarity of water in the open seas or lakes in not assured.  
As the preferred alternative we chose to perform this testing in a facility of 
the U.S. navy called the propulsion noise test facility located at the 
naval underwater warfare center in Newport RI. (see Fig. \ref{pntf}).

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/pntf}
\includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/pntf-2}
\end{center}
\caption[Propulsion Noise Test Facility (PNTF) at the Naval Undersea Warfare Center in Newport RI.]
{Propulsion Noise Test Facility (PNTF) at the Naval Undersea Warfare Center in Newport RI.
Photograph of PNTF on left, schematic of PNTF showing the storage vessel and other support 
facilities on right.} 
\label{pntf}
\end{figure}  

The facility consists of a 15 meter diameter spherical steel vessel with capacity of 
500,000 gallons of water. This vessel can be pressured to 6.9 bar at the center 
of the vessel. By simulation we have established that the facility satisfies 
the requirement of both being large enough to cause a shock event and to 
allow measurement of the shock event upto 10 ms.  
The vessel has two ports for entry. One of them is 48 inch 
across. The port opens onto an inside deck which we can use to place 
the PMTs and other apparatus for testing.  

There have been several visits to the PNTF. BNL and NUWC have 
entered into  a cooperative 
research and development agreement (CRADA) for the use of this facility. 
The PNTF has not been used for 17 yrs. After a considerable maintenance, 
it is back to work and several testing were performed on December 2010.  

\underline{\bf Schedule of testing and characterization } 

After the refurbishment of PNTF, the facility 
is fully operational in October 2010.  The pressure vessel facility at BNL
has been operational for several years, but now it needs to be upgraded to 
have  more controlled pressure increase. This will become operational in 
October 2011. The testing at these two facilities as well as the work 
at Alfred must be integrated with two critical decisions: the 
PMT size and shape, and whether the PMT should be enclosed in a pressure shell.  
The milestone schedule is shown in table~\ref{milepmtmech}.

\begin{table} 
\begin{tabular}{l|c|l}
Task & Quantity &  Completion Date \\
\hline  
PNTF operational &   & Sep. 30, 2010 \\
Glass testing  &  & Oct. 30, 2010 \\
BNL Vessel upgrade &   & Nov. 15, 2010 \\
PNTF Phase I testing complete & 2 PMT & Dec. 15, 2010 \\ 
BNL Pressure tests series 1 & 20 PMT & Jan. 17, 2011 \\
Glass and lifetime analysis 1 & & Feb. 2011 \\
Modeling and analysis &  & Aug. 15, 2011 \\
PNTF Phase II & 4 PA & Oct. 10, 2011 \\
Decision on PMT size & & Nov. 7, 2011 \\
BNL Pressure tests series 2 & 50 PMT &   Nov. 10, 2011 \\ 
Analysis of PNTF and BNL test data & &  Jan. 15, 2012 \\
PNTF Phase II & 4 PA & Mar. 15, 2012 \\ 
Decision on PMT enclosure (pressure shell) &  & Apr. 15, 2012 \\ 
BNL pressure tests series 3 & 200 &  Jan. 15, 2013 \\
PNTF Phase III PIU test & 2 PIU & Mar.15, 2013 \\
Decision on total shell versus back-shell &  & Aug. 15, 2013 \\
PNTF Phase III Final & 2 PIU & Oct. 15, 2013  \\
\end{tabular}
\caption{  Milestones for PMT mechanical characterization 
\label{milepmtmech}}
\end{table}

We have planned the PNTF testing in three phases: 
\begin{enumerate} 

\item  The purpose of phase I at PNTF is to establish that the 
facility is indeed appropriate for our use. In this test, PMTs will be 
imploded at static pressure of 5.8 bar. The implosion will be induced by 
a steel hydraulic device on the dome of the PMT which will have 
water proof bases and will be held in a prototype holder. 
The pressure field and motion of the water around the PMT will be measured 
using blast sensors (model 138A01 by PCB piezoelectronics) 
 read at 1 MHz. The event will be captured using fast motion cameras from 
two angles at a rate of 1000 frames per second.   
The PMT tests will be preceded by dummy bulbs to tune all the instrumentation 
before the final tests.  

\item The purpose of the phase II tests will be to obtain sufficient 
data on shock waves properties as a function of different conditions: these include 
PMT size and model, static pressure, location of the break and the effect of 
additional structural materials near the PMT. This testing will require 
implosion of several bulbs and with a near final design for the PMT assembly (PA).
The PA may include a prototype reflector or a representative device. PA may also 
include  initial design for  chain reaction mitigation such as an acrylic shell or 
a partial acrylic shell.    The data from these tests will be evaluated against 
two simulations: a 2D model of the shock wave generation as well as a 3D hydrodynamic 
model.    The models will be adjusted to reproduce the data as closely as possible 
and the nature and intensity of the shock at various distances will be evaluated.  

\item  The purpose of the phase III tests at NUWC will be to test the initial PIU 
assembly in a realistic   environment.   The PIUs will be assembled from PAs with 
near complete design for the PMT encapsulation and support structure.  
One of the PMTs will be mechanically induced to implode and the resulting 
cascade, if there is a cascade, observed with fast motion cameras and 
blast sensors.  It is expected that we will need two initial  tests with some conditions
varied to get good data. As an example, when the SuperK incident was 
reproduced a total of three tests were performed. After the two initial 
tests in the spring of 2013, there will be two final tests with the final design 
of the PIUs for verification.    It is anticipated that  
these final tests will also include other support structures such as 
the water-tight liner and cable assemblies.  

\end{enumerate} 

\underline{\bf Phase I NUWC Test}

In the Phase I stage, two 10 inch Hamamatsu PMTs have been conducted in two implosion tests
on December 16th and 17th, 2010 in PNTF.

The test stand was installed in a specified location near the center of the PNTF sphere. The PNTF
has a grated work platform about three feet below the center line.
There is also a large I-beam with a trolley for installation of a hoist for handling heavy equipment
or test items. ``Unistrut'' and PVC pipe was used to hold the PMT support fixture and hydraulic
piston assembly, underwater lights and the high speed cameras, etc.
Fig. \ref{fig:naval-1} shows the PMT setup structure and the sensors around the PMT.

\begin{figure}[ht]
 \centering
  \includegraphics[width=0.6\textwidth]{volume-4-WCD/figures/naval-1}
  \caption{Test stand with PMT and instrumentation installed}
  \label{fig:naval-1}
\end{figure}

Seven PCB Tourmaline Underwater Blast ICP Sensors (model 138A01 and 138A02) were
used in the tests. Six of them were mounted on the PVC piping frame, the remaining one
was mounted on the PMT support plate. Each sensor was connected to a PCB (model 481A-050-080)
Signal Conditioner. The output from the signal conditioner were routed to either a TEAC Integrated
Recorder (sample rate 200kHz/channel) or an IO Tech Wavebook (sample rate 500kHz/channel).

A plot of the pressure time history of one sensor (ACC5) is shown in Fig. \ref{fig:pressure-time-dec16-acc5}.
At time ``T0'', the sensor detected the hydraulic cylinder's force as the glass started to crack.
 After about 1 ms and at time ``T1'', the PMT collapsed, high pressure water started to rush in and
 compressed the low pressure gas in the PMT. The sensor detected the sudden drop of the water pressure
and then, as the collapse-phase ended when the gas reached it's minimum volume (closure).
At that moment the velocity of the water become zero. The hydrostatic pressure used in these experiments
caused the water to achieve a very high velocity during the collapse-phase. Upon closure of the gas volume,
the rapid change in water momentum caused compression of the water, and then a radial pressure wave (``T2'').
The pressure wave propagated toward the pressure vessel wall and then was reflected back toward the
center (``T3'').

 \begin{figure}[ht]
  \centering
    \includegraphics[width=0.6\textwidth]{volume-4-WCD/figures/sensor-500KHz-Dec16-ACC5-discription}
    \caption{The pressure time history of the PMT R0249 implosion recorded by blast sensor ACC5}
  \label{fig:pressure-time-dec16-acc5}
 \end{figure}

Fig. \ref{fig:pressure-time-dec16-4accs} shows the pressure and impulse time histories for sensor ACC1, ACC2,
 ACC3 and ACC4, which were oriented around the ``equator'' of the PMT and placed at the same distance from
the PMT. During the collapse-phase, the pressure time histories of sensors ACC1-4 are very similar.
ACC1 and ACC2 have almost the same peak pressure time, while ACC3 and ACC4 are also almost identical.
It is often useful to integrate the dynamic pressure with respect to time to calculate the impulse, $I$,
which is a measure of the momentum imparted to the water as the pressure wave passes through it.
Note that the dynamic pressure is obtained by subtracting the hydrostatic pressure from the absolute pressure,
so that at t=0, the impulse is zero. For time, t, between 0 and 10 ms, the pressure time history was
integrated between 0 and t. The strength of the positive portion of the pressure pulse is the difference
between the maximal impulse (occurring at about 8 ms) and the minimum impulse (occurring at about 4.7 ms).
 Although sensors ACC1, ACC2, ACC3 and ACC4 have the same distance from the PMT, they have quite different
peak dynamic pressures (up to about 50\%). However, they have very similar impulse intensities $I$ (15\%).
 Of particular note, for those recorded in the same data recorder, the impulse difference is only about 6\%.
 This means that the momentum imparted to the water in the four directions is uniform, even though there is
some local variation of the pressure time histories.

\begin{figure}[ht]
  \centering
    \includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/Dec-16-same-Sensors-Pressure}
    \includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/Dec-16-same-Sensors-Pressure-Integral}
    \caption[The pressure and impulse time histories of blast sensors]{The pressure time histories of the PMT
R0249 implosion recorded by four blast sensors on left. The impulse time histories of the PMT R0249 implosion
recorded by four blast sensors on right.}
  \label{fig:pressure-time-dec16-4accs}
 \end{figure}

Several of principal characteristics of the pressure pulses for seven blast sensors are listed in Table
\ref{table:pmt-dec-16}. One of the main characteristics of the pressure pulse is that all the seven sensors
 exhibit a similar collapse pressure time duration(T2-T0), of about 5.6 ms, although they are located at
different distances from the center of the PMT, so this pressure time duration is only related to the PMT
collapse process itself. If we calculate the relative maximum peak pressure time differences between these
sensors, they are very consistent with the speed of sound in water at 25 degrees Celsius, about 1497 m/s.
Another main characteristic of the pressure pulse is related to the impulse. The impulses for these sensors
show a clear $1/r$ relationship with respect to the distance from the PMT, $r$.

\begin{table}[ht]
  \begin{tabular}{c|c|c|c|c|c|c}
    \hline
    sensor & dist(mm) & T0(ms) & T2(ms) & T2-T0 (ms) & $P_{peak}$ (psi) & impulse (psi*ms) \\
    \hline
    ACC11 & 152 & 0.000 & 5.570 & 5.570 & 801.6 & 150.0 \\
    \hline
    ACC5 & 482 & 0.260 & 5.800 & 5.540 & 300.2 & 37.8 \\
    \hline
    ACC1 & 521 & 0.260 & 5.785 & 5.525 & 426.9 & 38.0 \\
    \hline
    ACC2 & 521 & 0.245 & 5.780 & 5.540 & 488.3 & 43.2 \\
    \hline
    ACC3 & 521 & 0.235 & 5.830 & 5.595 & 287.2 & 35.8 \\
    \hline
    ACC4 & 521 & 0.245 & 5.825 & 5.580 & 410.0 & 36.3 \\
    \hline
    ACC6 & 991  & 0.560 & 6.150 & 5.590 & 169.2 & 20.3 \\
    \hline
  \end{tabular}
  \label{table:pmt-dec-16}
  \caption{Pressure Sensor Response for PMT-R0249}
\end{table}

In order to check the repeatability of the test, another PMT implosion test was implemented for PMT R0284 on
December 17th, 2010. The set-up remained the same as in the first test. The result of the second PMT test is 
consistent with the first test.

\underline{\bf Mechanical Simulations } 

As explained above, the testing plan needs to be accompanied by
simulations.  We are planning on both calculations of stresses in
the PMT bulb with standard ANSYS tools as well as hydrodynamic simulations.

The stress calculations in the PMTs require detailed information regarding
the tube geometry. We have performed a set of detailed measurements on
6 R7081 and several Photonis and ETL  tubes to understand the variations in glass thickness and
the shape of the tube.  We have also obtained detailed drawings of the
glass bulbs.  Initial results show that the stresses in the neck and dome
transition area can be high (as much as a factor of 2 above the simple
spherical model). We are communicating with the vendors to understand
how to reduce these stresses by either changing the shape or making the region
thicker.

The hydrodynamic simulations present a must larger challenge. Partly because
the  implosion collapse and the shock pulse are a complex problem
requiring details of the glass, the motion of water, a model of all the material
that gets compressed as well as all the anisotropies present in the
PMT.  The relatively simple 2D simulations presented earlier give us
a basic understanding of the process, but the numerical value of the
peak pressure in the shock wave has a very large error. For example,
the simulation performed for SuperK after the accident over-predicted the
peak pressure in the shock at 50 cm from the 20 inch tubes to be 13 Mpa, but
was measured to be 5.6 Mpa. The time scale for the generation of the shock was,
however correct.

%Furthermore, we also will need to understand how the shock wave is modified
%by the PMT support structure and how it gets transmitted to the neighboring
%PMT.   We have consulted experts in such modeling and have learned that
%the shock generation will require experimental input, but the shock
%transmission could be simulated reliably with various mechanical modeling
%codes. We will solve this problem with 3-prong approach: the 2D simulations
%with specialized (DYSMAS~\cite{DYSMAS})
%code will be tuned to obtain the shock pulse, the transmission of the shock
%pulse will be studied using ANSYS based code or specialized code
%using LS-DYNA. A complete simulation of the PIU behavior with
%these tools will be expensive because it requires expert manpower as well as
%considerable computer time.

In an effort to develop a computational tool that can be utilized to
optimize the photomultiplier tube arrangement in the LBNE experiment,
an elaborate numerical analysis was conducted. The main objectives of
this multi-faceted effort were (a) the benchmarking of a physics-based
implosion model against data from relevant past studies, (b) the
evaluation of the capacity strength of the selected PMT in
coordination with specific, new hydrostatic tests and the
understanding of an implosion-induced shock-wave, and (c) the
prediction of the shock field around the imploding PMT under the LBNE
ambient parameters to be simulated in the NUWC large-scale tests.

The basis for the numerical models used in addressing the various
experiments as well as appropriate sensitivity studies is the
Arbitrary Lagrangian Eulerian (ALE) formulation provided by the
LS-DYNA explicit code which enables the study of both fluid and solid
parts and their interaction under highly non-linear processes
associated with the PMT implosion. The capabilities of the TrueGrid
software were utilized to generate an accurate 3-D description of the
various test configurations. The analysis performed are considered
``blind'' predictions due to the fact that (a) they were all performed
ahead of the experiments and (b) it was necessary to make certain
assumptions regarding the equation of state (EOS) constitutive and
glass fracture relations governing the PMT glass
material. Specifically, the properties of float silica glass adopted
into the Johnson-Holmquist constitutive model were used to describe
the PMT glass wall in the implosion simulations.

Borosilicate glass spheres of 7.62~cm outside diameter and 0.762~mm
nominal thickness were imploded with the help of a mechanical device
in 6.996~MPa hydrostatic and 101.3~kPa (1~Atm) inner pressures while
implosion-induced pressure pulses were recorded at 10.16 cm by
pressure sensors. These tests were used as the benchmark frame for the
3-D ALE computational model being developed for the LBNE PMT implosion
studies. Fig.~\ref{fig:pred-sphere} depicts the comparison of the
numerical model predictions and those recorded during the actual
implosion tests. Additional benchmark studies were performed
addressing the ''bubble'' collapse/oscillation problem for which
analytical and semi-analytical solutions exist and for which the role
of the glass is eliminated thus representing the ''limiting'' case in
terms of generated peak pressures.  For both the glass sphere
implosion experiments and the bubble collapse problem the numerical
model accurately predicted both peak pressures and arrival times thus
providing confidence in analyzing the more complex PMT implosion
issue.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/prediction1}
  \includegraphics[width=0.49\textwidth]{volume-4-WCD/figures/prediction2}
  \caption{Predicted and recorded pressure pulse following the implosion of borosilicate glass sphere}
  \label{fig:pred-sphere}
\end{figure}

Following the benchmarking of the numerical processes and the
validation of the BNL small-scale hydrostatic tests, a numerical model
was developed to analyze the PMT implosion tests within the large
pressurized vessel at NUWC facility with a hydrostatic pressures of 88
psi and the implosion of the PMT was initiated with a mechanical
device. By taking advantage of the symmetry plane a model consisting
of a total of $\sim$ 2,240,000 elements representing the PMT glass
structure (Lagrangian) and all the fluid volumes (Eulerian) was
developed. To ensure that the pressure driver of the implosion is not
lost following the fracture of the PMT wall, a large volume of the
surrounding water was used along with radiating boundaries at the
water volume edge.  The implosion analysis consisted of an
initialization phase establishing the state of stress in the PMT wall
followed by a transient phase capturing the glass damage initiation
and the subsequent implosion. The duration of the glass implosion was
of primary interest, given the ambient pressure of 88 psi and the
subsequent pressure intensity and spatial attenuation.  An Analysis
time of 6 ms following the PMT fracture initiation was used.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.45\textwidth]{volume-4-WCD/figures/sim_nuwc1}%
  \includegraphics[width=0.45\textwidth]{volume-4-WCD/figures/sim_nuwc2}

  \includegraphics[width=0.45\textwidth]{volume-4-WCD/figures/sim_nuwc3}%
  \includegraphics[width=0.45\textwidth]{volume-4-WCD/figures/sim_nuwc4}
  \caption{Simulated shock initiation and propagation during the NUWC PMT implosion tests.}
  \label{fig:nuwc-simulation}
\end{figure}

Fig \ref{fig:nuwc-simulation} depicts the initiation of the shock within the volume of the PMT followed by the outward propagation. 
The analysis indicates that the collapse process for the 88 psi ambient pressure will take approximately 4.425 ms from the moment 
of wall fracture initiation. 

The simulated pressure pulse intensities as well as their arrival at locations in the surrounding volume where pressure sensors were 
to be placed during the actual tests are compared with the real tests. Shown are pressures near the mechanical device used to initiate 
the fracture that is close to the PMT wall (ACC11) and at $\sim$ 0.5 m (ACC1, ACC2, ACC3 and ACC4) radial distances from the center of 
the PMT. The simulated pressure time histories agree with the real test data fairly well. There are some differences between the real 
tests and the simulation. In the simulation, sensors' pressure readings drop dramatically at the beginning of the implosion, while it 
is quite smooth for the real data. And the duration of implosion for the simulation is always shorter than the actual tests by around 
0.5 ms. These differences are most likely related to differences in the properties of the glass. Because of lacking of Borosilicate 
glass properties for the simulation, normal silica glass properties are used in the simulation. It seems that during the cracking phase 
of Borosilicate, the glass still stay somewhat intact and the pressure didn't drop dramatically. However the normal silica glass cracking 
speed is very fast, so a big drop in pressure is shown in the simulation. Another main difference for the real tests and the simulation 
is in the peak pressure value. The simulated peak pressure is relatively smaller than the actual test data by about 90 psi. Since the peak 
pressure is also strongly correlated with the glass cracking, it may also related with the property of the glass. Generally speaking, 
current simulation describes the PMT implosion process fairly well, even when different glass properties are used.

\begin{figure}[ht]
  \centering
  \includegraphics[width=\textwidth]{volume-4-WCD/figures/Data-MC-Comparison-Dec-16}
  \caption{Predicted pressure pulse arrival times and intensities at the location of pressure sensors during the NUWC implosion tests.}
  \label{fig:predict-nuwc-sensors}
\end{figure}

\end{appendices}





==> volume-4-WCD/pmt-mechanical.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

%Turn this into an appendix
%\subsection{Mechanical Characterization}
%\label{subsec:v4-photon-det-pmt-mech}

\subsubsection{Objectives}

 The primary objective, and the key challenge, of the mechanical characterization 
program is to minimize the risk of single-PMT implosion and eliminate the risk of a catastrophic chain reaction of PMT implosions.

The ability of the PMTs to withstand the water-column pressure at maximum depth (about 5.8~bar at $\sim$60 m) is crucial to the success of the experiment. Implosion of a single tube could lead to a cascade failure of neighboring PMTs, resulting in a long downtime and hefty expense to replace the tubes, and to degradation of the experimental data if the PMTs cannot be replaced.  Prior to ordering, therefore, sample tubes will be subjected to pressures equivalent to or greater than those at the deepest location in the water tanks.  Cycling pressure tests will also be performed.  Depending on the availability and cost of testing facilities, a random sampling of PMTs may also be tested during production.

Two options exist regarding placement of the PMT in the water.
Our reference design places the PMTs with the glass bulb in contact with the water; they are therefore subjected 
to the full hydrostatic pressure. In this case, the HV base must be encapsulated to be water-tight.  
Alternatively, 
 the PMT can be completely encased in a pressure housing that prevents contact
between water and bulb; in this case the PMT itself does not need to withstand the full static load.

We will only discuss our reference design configuration here. The goals of the PMT mechanical characterization program are summarized below.
%\fixme{It used to say "the requirements are:"  If these are requirements, how come they're not in the req doc?}

\begin{enumerate} 
\item Ensure that the maximum failure rate by implosion does not exceed
$\sim$0.5\%/yr, assuming all other failure mechanisms are negligible. This translates to 90\% of
the tubes remaining ``alive'' over the lifetime of the experiment, in accordance with the science goals. 
\item Ensure that, in case of a PMT implosion, neither the resulting inward motion of the water nor the following outward shock wave causes implosion failures of any neighboring PMTs.
The total energy released in an implosion would be the
pressure times volume of the PMT, $P \times V$. For $P =$5.8~bar and $V =$5~liters
 (for a typical 10-in diameter PMT), the energy released will 
be about $\sim$3000 joules.  This energy will go mostly into the kinetic energy
 of the water around the PMT. It will first convert into inward motion of the 
water and then a shock wave transmitted outwards when the inward 
flow is interrupted by the impact of the water on itself. 
\item Eliminate the risk of a chain reaction causing failure of a substantial fraction of 
PMTs.  
%\item Eliminate the possibility of correlated PMT failures in a local area of more than nine PMTs.  
\item Study and eliminate risks of an individual PMT implosion introducing failures in 
neighboring support structures, active structures such as 
cables, or the water-containment liner.  
\end{enumerate} 


\subsubsection{Program Components} 

The mechanical testing program has two components: understanding 
the static load performance of the PMT and understanding the performance of 
the completely assembled system with PMTs, cables and support structure 
under the dynamic conditions of implosion.  

The program will be carried out in phases and each phase will be integrated 
with PMT specification, the procurement plan and 
the detailed design work on the PMT Assembly (PA).  

It is extremely important to start this program early in the conceptual 
design phase. Early results will determine if the PMT has to be completely 
encased or partially encased to prevent a chain reaction event. 
The results will also inform us with regards to the optimum distance between 
tubes and the optimum size of the tubes.  

In Appendix~\ref{appx:pmt-char} we describe the resources identified to start on 
this process during the CD-1 phase, and our current vision of how the 
program will evolve over time.  



==> volume-4-WCD/pmt-opt-elec-req-appx.tex <==
\begin{appendices}
\chapter{PMT Optical and Electronic Requirements}
\label{appx:pmt-optoelec-req}

\section{Timing}

Figure~\ref{fig:timing} shows a plot of time-of-flight residuals for 6.1~MeV
$\gamma$ rays (from an $^{16}$N source) for Hamamatsu R1408 PMTs in
the Sudbury Neutrino Observatory (SNO). Many of the features discussed
in this section are indicated in the figure.
\begin{figure}
\begin{center}
\includegraphics[height=0.4\textheight]{volume-4-WCD/figures/timeresid.pdf}
\caption{Time-of-flight residuals for $\gamma$ ray events from an  $^{16}$N
calibration source in SNO.  \label{fig:timing}}
\end{center}
\end{figure}


\subsection{Transit Time Spread (TTS)}

  The position resolution of events in the detector  will depend primarily on
the relative timing of the PMT hits.  The narrower the spread in hit times for
an equidistant, prompt source of light, the narrower the position resolution of
events in the detector.  At low energies, water Cherenkov detectors have
achieved position resolutions of roughly 20~cm for events with 40 or more hits,
using PMTs with roughly 1.6~ns transit time spreads (TTS), measured as the
Gaussian width ($\sigma$) of hits in the prompt peak (shown above in
Figure~\ref{fig:timing}).  For our WCD, 40 hits would correspond to roughly 10
MeV, depending on PMT coverage and efficiency.  
To get down to 7~MeV, where perhaps a solar day/night
asymmetry measurement could be made, and to keep the same vertex resolution as
has been achieved in previous experiments, we require the same average
$\sigma_t= 1.6$~ns yielding a one-dimensional position resolution of
$\sqrt{40}/\sqrt{28}(20{\rm cm}) \sim 24$~cm, well within the high-level 30~cm
resolution requirement for the experiment.

\subsection{Latepulsing}

	`Latepulsing' is a phenomenon associated with the collection of
electrons by the PMT.  In some cases, an electron creates a photon at the first
dynode that then travels to the photocathode and creates a second PE.  More
commonly, the PE elastically scatters off of the first dynode, and the time
taken on its return path delays the pulse arrival time.  

	These latepulses either reduce the number of hits that are usable or,
get confused with hits from scattering and reflections when used in
reconstruction.  So we treat these late hits as losses of light, and require
the fraction of latepulses, taken as the integral from 5$\sigma$ after the mean
of the prompt peak out to 80~ns, to be less than 5\% of the events in the
prompt-timing peak.

\subsection{Prepulsing}
	Prepulsing is caused when a photon passes through the photocathode and
strikes the first dynode directly.  In modern tubes, these are much rarer than
latepulses, so it is reasonable to set the requirement that the fraction of
prepulses, taken as the integral from $-2\sigma$ before the mean of the prompt
timing peak to $-100$~ns, to be less than 1\% of the total number of pulses in
the primary timing peak.

\subsection{Afterpulsing}

	Afterpulsing is caused by the ionization of residual gas atoms in the
PMT, and because of the slow travel time of the resulting ion toward the
photocathode, they tend to come at timescales that are more than 1$\mu$s after
the prompt light.  Afterpulses are less dangerous than latepulses, because they
do not directly affect the position resolution of most events of interest.
They can, however, pile-up with delayed events (e.g.  Michel electrons) and if
the probability of occurrence is more than 5\% per hit, they can 
muddle the identification of delayed events.  In a sense, they cause the
detector to be effectively dead for a few $\mu$s.  Gas leakage into
the PMTs must be small enough that the change in afterpulsing rate, after
storage for five years or so, does not change noticeably. The leakage could be
tested by immersing several PMTs in a helium bath for several months, and
testing the afterpulsing rates at several times during the immersion.

\subsection{Double Pulsing} 

  Double pulsing (or `echo pulsing') is the occurrence of a second pulse
following a prompt (in-time) PMT pulse, when only a single photon has hit the
PMT. The exact mechanism that causes the phenomenon is not known, but it may be
the result of a prompt secondary electron created by a photoelectron scattering
off of the first dynode, that is then followed by the primary photoelectron
coming as a latepulse.

  Double pulsing is not a problem for integral electronics if it occurs with
every pulse, but if occurs sporadically  it can lead to difficulties in
counting photons and therefore smear the detector's energy resolution.  In
addition, for the time-over-threshold electronics described in
Section~\ref{subsec:v4-elec-readout-frontend-reqs-n-specs}, double pulsing will
make the separation of multiple photons more difficult.  We require the
probability of double pulsing to be on average $<$5\%.

\section{Pulse shape}

	The pulse shape of the PMTs will affect the timing, the ability to
separate multiple photons (even in the most sophisticated electronics scenario)
and the ability to see signal above possible pick-up and noise levels on the
cable and within the electronics.  Perhaps the most stringent requirement comes from the
last item, given the dispersion of the PMT signal along the cable lengths expected
for LBNE.  As shown in Figure~\ref{fig:pulses}, the dispersion tends to stretch
\begin{figure}
\begin{center}
\includegraphics[height=0.4\textheight]{volume-4-WCD/figures/pulse_cable.pdf}
\caption[Effect of 150 m of cable on PMT output pulse.]
{Effect of 150 m of cable on PMT output pulse.
The pulse out of a Hamamatsu R7081 (red trace) is compared to the same pulse
after it passes through a $\sim$150~m cable (blue trace), roughly that 
expected for LBNE-WCD.\label{fig:pulses}}
\end{center}
\end{figure}
out the fall time of the pulse (blue trace compared to red trace), thus
reducing its overall amplitude for a given amount of charge. Simple
measurements on ``LBNE-length'' cables with no compensation
showed that the fall time after passing through the cable
can be as long as 40~ns or so, while the risetime is roughly 4~ns, not much
longer than that of the PMT itself.  Thus at a gain of $10^7$, the peak
amplitude of a pulse with 0.25 PE of charge is about 1~mV, just
above where we might expect the noise level to be.  A faster intrinsic pulse
from the PMT will lead to a narrower (and higher amplitude) pulse at the end of
the cable.  Under the assumption that we will trigger on PMTs at 0.25~p.e.
threshold, and a gain of $10^7$, a reasonable requirement for the risetime at
the PMT (measured with a cable whose length is $<1$~m) is 4~ns with a fall
time of 12~ns.

\section{Charge}
	Figure~\ref{fig:qspec} shows the single PE spectrum for a
Hamamatsu R7081 PMT, with some of the terms of this discussion annotated.
\begin{figure}
\begin{center}
\includegraphics[height=0.4\textheight]{volume-4-WCD/figures/charge_spectrum.pdf}
\caption{Single PE charge spectrum for a  Hamamatsu R7081.
\label{fig:qspec}}
\end{center}
\end{figure}

\subsection{Peak-to-Valley Ratio (P/V)}
   The single-PE-charge response of the PMT has several effects on
the eventual analysis of data.  The photon-detection efficiency for each
electronics channel depends on where the individual channel thresholds can be set, which
in turn depend on the shape of the single-PE spectrum.  The lower the thresholds
can be set, the more photons are detected and hence the requirements for
position and energy resolution are more easily satisfied. In setting thresholds,
the competition is between detection efficiency and PMT-noise rate. Typical
threshold settings are at 0.25 of the single-PE peak, but a lower
threshold increases the detection efficiency.  The
characteristic that most directly determines threshold setting is the depth  of
the `valley', where the low-charge side of the primary single-PE
spectrum runs into the much lower-gain spectrum that falls roughly exponentially
from zero. For modern PMTs, the requirement of a typical peak/valley ratio of 2
or more is reasonable and ensures that the detector can be run at a threshold
of 0.25 PE, if the level of electronic noise and pickup can be kept low enough.

\subsection{Single-Photoelectron-Charge Resolution (Charge Width)}
	The single-PE-charge resolution is typically measured as the
distance of the `high half point' from the peak of the single-PE
spectrum.  The resolution is dominated by the number of secondary electrons
produced at the first dynode. Narrower resolutions (higher first-dynode
multiplicities) enable better separation of multiple photons, but usually only
specially designed (and small-area) PMTs are able to resolve two photons from
one. Nevertheless, single-PE-charge resolutions of roughly 50\%
(taken as a fraction of the single-PE peak charge) are possible, and
will allow separation of one PE from three or more, and at least some handle on
differences between one and two.  

\subsubsubsection{High-Charge Tail}
	Beyond the half-width of the single-PE peak, some PMTs
exhibit a long tail on the single-PE spectrum, beyond what would be
expected from a simple Polya distribution.  This long tail may be associated
with electrons that strike areas of the PMT (such as a focusing grid) on their way to the first dynode.
 This long tail can make it difficult to determine if
a PMT with `too much charge' is indicative of a problem (such as a flasher PMT).
Most modern PMTs do not exhibit this long-tail, nevertheless we require that the
PMT selected for LBNE has fewer than 1\% of its single-PE hits beyond 3$\sigma$
of the single-PE peak.
  
\section{Gain}
	As discussed above, we would like to trigger on single-PE
pulses at an equivalent threshold of 0.25 PE.  This threshold requires that
the peak of the single-PE pulse be above the electronic-noise level,
including sources of pickup.  If we assume that this noise level is around 1~mV,
and that a worst-case cable dispersion and attenuation effectively reduces the
amplitude of the pulse by a factor of 3 or so (based on measurements with long
cables), a gain of $10^7$ or more is required to trigger at the desired level.

	Many of the events in LBNE will produce large numbers of photons, and
very high-energy, through-going muons may lead to a thousand or more PEs in
each PMT.  To simplify the data analysis, we require that the response of the
PMT has an integral non-linearity no larger than 10\% from 1 to 1000
photoelectrons, for narrow (Cherenkov-like) pulses.


\section{Dark Current}
  PMT dark current, due to things like the thermal emission of electrons from
the photocathode and dynodes, leads to pile-up of noise hits with hits due to
Cherenkov light.  Higher noise rates increase the rate of accidental
coincidence events for a given trigger threshold, force the trigger threshold
higher (with a consequent slow turn-on of the trigger efficiency curve), or
degrade the energy and position resolution for high-energy events.  At the
detector's ambient temperature, we require the average noise rate to be no
higher than 1.5 kHz at the nominal threshold and gain chosen to run the
experiment, for a 10'' high quantum efficiency PMT.  We note that this is not a
specification delivered to a manufacturer, but a statement about the behavior
under our expected running conditions.  We do not include here the additional
noise that is caused by the radioactivity in the water and other PMTs.


\section{Wavelength Response}

  Under the assumption that we do not use light concentrators or other
light-enhancement techniques, the wavelength response of the PMT should cover
the wavelengths that ultra-pure water will pass.  The light attenuation of the
water is minimal for wavelengths around 420~nm  and some
samples have been known to approach the Rayleigh scattering limit at that point
(with an attenuation length of roughly 100~m). By 350~nm, however, the
attenuation length (including both extinction and scattering) drops below 100~m
and therefore for LBNE these wavelengths will be noticeably attenuated.
Weighting by the $\sim 1/\lambda^2$ Cherenkov spectrum, this results in a peak
response near 400~nm. Therefore we require the efficiency of the PMT as a
function of wavelength should peak in the region 370-420~nm.



\section{Spurious light emission}
  Nearly all water Cherenkov experiments have had problems with the spontaneous
emission of light from PMTs.  The behavior of flashing PMTs is very different
for different PMT types, and it is likely that the sources of these events are
different for the different models.   In \superk{}, flasher PMTs `turn on' for
a while and become worse at which point the PMT needs to be turned off for some
amount of time.  In SNO, all PMTs exhibited the flashing behavior albeit at low
rate: roughly 1 flash emitting 500 photons or more per week for each PMT,
resulting in a detector-wide rate of about 1/minute.  In SNO, a suite of cuts
(including reconstruction) were developed to remove these events from the final
solar-neutrino data set, at a level that was below one event
in several years' running.  In LBNE, the number of PMTs will be much larger, so
that for a given module perhaps 50,000 will be used, resulting in a flashing
rate that for SNO-like flashers would be as high as once every 10 seconds.  To
keep the rate in the final data set as low as was achieved in SNO, under the
assumption that a set of cuts can be developed as efficient as those SNO did,
we require the PMTs to spontaneously emit light of intensity above 500 photons
no more often than 1/month.


\section{Stability}

\subsection{Gain and Efficiency}
	Systematic uncertainties on detector position and energy resolution will
depend on how well changes to the detector's behavior can be tracked by
calibration sources.  Although in principal PMT changes can be tracked very
accurately, to do so continuously may create a high overhead on the overall data
set. We therefore require that the gain and efficiency of the PMTs drift by no
more than 3\%/year, at a fixed high voltage.

\subsection{PMT Timing}
	Changes to PMT timing are not expected, but changes in latepulsing or
afterpulsing should not be larger than 10\% of their initial values.

\subsection{Noise Rate}
	Likewise, for fixed temperature and high-voltage settings, the average
noise rates of individual PMTs should not fluctuate by more than a factor of
two, for averaging periods of a month,
after the initial cool-down period. 


\section{Robustness}
\subsection{Temperature Excursions}
	The PMTs may be exposed to several events which may affect their
efficiency.  During storage or transport, while in the cavity before and after
submersion, the PMTs may be exposed to temperature variations of as much as 40$^\circ$C.  
We require that after such exposures, there be no permanent change to the
PMT efficiency or gain at a fixed high voltage, to better than 1\% and 10\%
respectively, and no permanent change to the PMT noise rate over 10\%.

\subsection{High Illumination}
Similarly, the PMTs may be exposed to high light levels, for example
during work inside the cavity or during assembly.  We require that after
exposure to the ambient lighting of the cavity during construction (with no
applied high voltage), there is no permanent change to the PMT efficiency or
gain at a fixed high voltage, at better than 1\% and 10\% respectively, and no
permanent change to the PMT noise rate of more than 10\%. We expect such
lighting to be within 10 times that of a standard office, or up to 1000
lumens/m$^2$.


\subsection{Seismic Events}
	During transport, construction, and after installation, the PMTs may be
exposed to vibration due to seismic or construction activity in the mine. We
require that after such events, events, there be no permanent change to the PMT
efficiency or gain at a fixed high voltage, at better than 1\% and 10\%
respectively, and no permanent change to the PMT noise rate over 10\%.
\end{appendices}

==> volume-4-WCD/pmt_radioactivity.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

{\bf Radioactivity}
\label{subsec:v4-pmt-radioactivity}

Natural radioactivity in the materials of the PA can give rise to multiple
PMT hits if the gamma rays from the radioactive decay produce
energetic electrons (via Compton Scattering) in the WCD water. In
water, the absorption length of 1--2~MeV photons is $\sim$20~cm %(ref http://pdg.lbl.gov/2011/reviews/rpp2011-rev-passage-particles-matter.pdf, fig 27-16) , 
so the two meters of buffer water between the PMT plane
and the fiducial volume effectively eliminate any of these energetic
photons from reaching the fiducial volume. However, the light produced
in the buffer region can cause multiple PMTs to trigger, potentially
driving up the trigger rate at low energy, or equivalently raising our
low energy threshold in the attempt to keep the trigger rate
manageable.

Fortunately, due to previous experiments that required low background
PMTs, the production of low activity glass, both by the selection of
glass type, and by the production process itself, has made the issue
much more tractable. The other materials used in the PA will also be chosen 
to minimize the natural levels of radioactivity.%\fixme{would be nice to have a reference here!}

The radioactivity in the PA needs to be smaller than
the activity we would expect to see in the
buffer volume coming from the natural radioactivity of the materials
in the wall of the WCD.  
%\fixme{need to get the spec used for our PMT}%ref(J. Felde, Docdb 966, http://lbne2-docdb.fnal.gov:8080/0009/000966/003/RadioactivBackground_Felde_LBNE.pdf)




==> volume-4-WCD/pmt_waterclarity.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

{\bf Impact on water clarity}

The PA and light collectors represent a significant fraction of the total surface area that is in contact with the water. 
It is therefore important that the chosen materials, and their handling (potential contamination of surfaces) not adversely affect the water's clarity. The clarity is
mathematically described by the wavelength-dependent attenuation length of the Cherenkov photons. It is composed of three quantities, the 
absorption length, the Rayleigh scattering length, and the Mie scattering length.  Rayleigh Scattering is a fundamental feature of light passage through a molecular medium,  most likely insensitive to relatively small levels of contaminants. However the absorption and Mie scattering lengths could be strongly dependent on these levels.

Leaching of contaminants from the materials of the PA and light collector could negatively impact the absorption length, thus reducing the total light yield at the surface where the PMTs are installed. All materials used in the PA and Light collectors will be tested to be compatible with the ultrapure water (see section~\ref{sec:v4-water-sys-mat-compat}). Although not directly related to clarity, leaching might also compromise the overall strength of the PMT glass envelope and impact the functionality of the other PA components.
 R\&D programs (see section ~\ref{subsec:v4-pmt-mech-glass-strength}) are underway to verify the robustness of our design. 

The addition of macroscopic particulates from dusty surfaces into the water will impact the Mie scattering length. An increase of photon scattering leads to a loss of prompt timing events (they will arrive late compared to non-scattered photons). The cleanliness specifications of the PA and light collector surfaces are under development (see section~\ref{subsec:v4-integ-integ-exp}). Their impact on the PA subtask, is on the level of surface cleanliness of the PA components when they are packaged  and shipped from our Integration Facility to the Installation Storage Facility (ISF) near the mine site. The level of necessary cleaning of the PA components in the PA assembly stage will depend on the cleaning that  will occur just before, during, or after actual installation of the PAs in the WCD.




==> volume-4-WCD/title.tex <==

\begin{center}
  {\LARGE Volume 4: Water Cherenkov Detector}

  {\Huge Conceptual Design Report} 
\bigskip

  {\Large \today}
\bigskip

  \includegraphics[height=5in]{volume-4-WCD/figures/WCD_image}

\end{center}

\newpage
\renewcommand{\thepage}{\roman{page}}
\setcounter{page}{1}

\setcounter{tocdepth}{3}
\tableofcontents

\newpage

\listoffigures

\newpage

\listoftables
\newpage

\renewcommand{\thepage}{\arabic{page}}
\setcounter{page}{1}



==> volume-4-WCD/water-cont-install.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.


\section{Installation (WBS 1.4.2.7)}
\label{sec:v4-water-cont-install}
Installation for all components (all have to write) Remember this is
not the installation labor itself but all the engineering and
supervision (EDIA) for it.

All group leaders should think about this and write about plans during
actual installation. We need to describe the installation process in
some detail.


\subsection{Requirements and Specifications}
\label{subsec:v4-water-cont-install-reqs-n-specs}

\subsection{Description}
\label{subsec:v4-water-cont-install-desc}



==> volume-4-WCD/water-sys-cooling.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.


\section{Water Temperature Control (WBS 1.4.6.4)}
\label{sec:v4-water-sys-cooling}

Chilling a volume of water inhibits the growth of micro-organisms
within it. Minimizing bacterial growth is very important for
maintaining adequate water purity in the detector. We will use
sterilization as a first step, but during recirculation, the detector
water will pass through a chiller unit designed to maintain the water
temperature at $13^{\circ}C$.

\fixme{Too early to describe chiller unit?}

It has been demonstrated that this temperature sufficiently inhibits
bacterial growth \fixme{a reference?? --- SuperK has demonstrated?}.
Experience with IMB detector which was operated in the 1980's has shown
that even if the detector water is turned over every month, organism
growth will occur if the temperature is too high.

As an additional benefit, chilling the water will reduce PMT
noise. \fixme{refer to plot of noise vs. T} Thermal modeling and water
flow patterns are discussed in section~\ref{sec:v4-water-cont-vol}. We plan
to use cold water taken from the surface as the exchange fluid in the
underground heat exchanger. The temperature of the water from the Deadwood
industrial water supply ranges between 3--15$^\circ$C.



==> volume-4-WCD/water-sys-drain.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.

\section{Water Draining (WBS 1.4.6.x)}
\label{sec:v4-water-sys-drain}

\fixme{Has WBS changed to include this? Let's fix number}

During the projected several decades-long operation of the detector
it may be necessary to drain the vessels for servicing or repair.
The drainage system will consist of the pumps normally used for recirculation
plus additional valves and piping to provide a mechanism for draining the
tank and transporting the water to the Underground Ground Waste Water Dump.

To preserve the Gadolinium option, the drainage system must
be capable of handling the full volume of water containing 0.1\% Gd.  Given
the large volume, the drainage system would include additional pumps in the
sump pit and piping to bring the water over to the shaft and up to the surface
for treatment. The output pressure and capacity of the pumps would be matched
to the piping and pressure control proposed in the shaft. \fixme{we should reference this -- I'll find it!}



==> volume-4-WCD/water-sys-operations.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.


\section{Water System Operations (WBS 1.4.6.x)}
\label{sec:v4-water-sys-operations}

\fixme{this is a little bit about water operations and a little about
consumables. Doesn't really seem to fit together.}

To complete a fill in the case of approximately 150~kTon total volume, we will use
about 400,000~lbs of water-softener salt, 800~ft$^3$ of U/Th-exchange
resin, 4000~ft$^3$ of deionizer-exchange resin and a number of
filters, UV lamps, etc. We estimate 400~man-hours of shift operation
for this procedure.

We intend to begin the recirculation of the detector water as soon as
filling begins. This will maintain the required water quality and
detector temperature during the fill.

During each year of operation, the recirculation system will require
2,400 cubic feet of both U/Th and mixed bed deionization resin. In
addition we will use about 400 40~in filters and 80 UV lamps. We
estimate the consumable cost to be about \$1.5M per year.


==> volume-4-WCD/water-sys-sump.tex <==
% PLEASE FOLLOW POSTED GUIDELINES!!

% Please see the two WCD CDR 'guidelines' writeboards in basecamp
% at https://lbne-doc.basecamphq.com/projects/4264327/writeboards
% One is for text, the other for images and figures 
%
% They are also available by building volume-X-dummy.tex.  You can
% look at the LaTeX source in that file and those under
% volume-X-dummy/ directory for examples.


\section{Water Sump System (WBS 1.4.6.5)}
\label{sec:v4-water-sys-sump}

It is likely that despite all our engineering efforts the detector
will leak small amounts of water. 
%Engineering practices specify that vessel leakage must be less than 0.05\% per day. At this level, a detector holding 130,000 tons of water will leak up to 17,000 gallons per day (or 70 tons/day) that we must handle. 
As discussed previously in section~\ref{sec:v4-water-sys-recirc}, we
have scaled from \superk\ to estimate this rate. Therefore, a detector
that holds \WCDweight\ of water is expected to leak approximately
2,000 gallons per day.  In addition, mine water from sources in the
surrounding rock and periodic usage of the underground reverse osmosis unit
will contribute to this waste water load.


Our sump system must collect the waste water, from both leakage and
the mine, and pump it to the mine disposal system. To ensure against
intermittent pump or electrical failure, we plan for
temporary storage of approximately two days worth of leakage \fixme{(or 15~m$^3$)}.

Our design calls for two sump pumps in a storage pit. One pump will
operate while the other is in standby mode.  \fixme{Describe concept
for sump pump and temp storage}


To preserve the Gadolinium option, the sump system must be capable of
handling water containing 0.1\% Gd. In this case, we would need to
treat the leakage water underground before rejecting the Gd-free water
to the mine's Underground Ground Waste Water Dump.

\fixme{and how do we propose to do this?}
\fixme{This needs to be described in the Gadolinium chapter and referenced here.}
